Adaptive Threshold-Driven Continuous Greedy Method for Scalable Submodular Optimization

Submodular maximization under matroid constraints is a fundamental problem in combinatorial optimization with applications in sensing, data summarization, active learning, and resource allocation. While the Sequential Greedy (SG) algorithm achieves only a $\frac{1}{2}$-approximation due to irrevocable selections, Continuous Greedy (CG) attains the optimal $\bigl(1-\frac{1}{e}\bigr)$-approximation via the multilinear relaxation, at the cost of a progressively dense decision vector that forces agents to exchange feature embeddings for nearly every ground-set element. We propose \textit{ATCG} (\underline{A}daptive \underline{T}hresholded \underline{C}ontinuous \underline{G}reedy), which gates gradient evaluations behind a per-partition progress ratio $\eta_i$, expanding each agent's active set only when current candidates fail to capture sufficient marginal gain, thereby directly bounding which feature embeddings are ever transmitted. Theoretical analysis establishes a curvature-aware approximation guarantee with effective factor $\tau_{\mathrm{eff}}=\max\{\tau,1-c\}$, interpolating between the threshold-based guarantee and the low-curvature regime where \textit{ATCG} recovers the performance of CG. This shows that the problem structure, as captured by curvature, determines the amount of coordination and communication required to approach full-CG performance. Experiments on a class-balanced prototype selection problem over a subset of the CIFAR-10 animal dataset show that \textit{ATCG} achieves objective values comparable to those of the full CG method while substantially reducing communication overhead through adaptive active-set expansion.

==> Algorithm_design_origional.tex <==
\section{Proposed Algorithm and Theoretical Guarantee}\label{sec:algo_theory}

We now introduce the proposed \textit{Adaptive Thresholded Continuous Greedy} (\textit{ATCG}) algorithm (Algorithm~\ref{alg:atcg}). The key idea is to regulate which elements actively participate in the greedy updates by maintaining dynamically expanding \emph{active sets} within each partition. Let the ground set be partitioned as $\mathcal{V}=\bigcup_{i=1}^N B_i$, where each partition $B_i$ contains the candidate elements associated with partition $i$. At each iteration $t$, the algorithm maintains an active set $A_i\subseteq B_i$ consisting of elements whose marginal gains are used in the greedy update.

In the classical continuous greedy algorithm, the ascent direction is obtained by solving
$
\max_{\vect{v}\in\mathcal P}\;\langle \vect{v},\nabla f(\vect{x})\rangle,
$
where $\mathcal P$ denotes the partition-matroid polytope. Under a partition matroid with budgets $\kappa_i$, this maximization decomposes across partitions and selects the top-$\kappa_i$ elements with the largest gradient values in each partition. For simplicity of exposition, we consider the case $\kappa_i=1$, in which case the oracle reduces to selecting the element with the largest gradient value in each partition, namely
$
\max_{j\in B_i} [\nabla f(\vect{x})]_{(i,j)}.
$
The algorithmic idea and the theoretical results extend naturally to the general case $\kappa_i>1$ by replacing this operation with a top-$\kappa_i$ selection rule.

To evaluate the quality of the current active set, the algorithm uses the following \emph{progress ratio} for each partition:
\begin{equation}\label{eq:eta_def}
\eta_i
=
\frac{\max_{j\in A_i} [\nabla f(\vect{x})]_{(i,j)}}
{\max_{j\in B_i} [\nabla f(\vect{x})]_{(i,j)}}.
\end{equation}
This ratio measures how well the best element currently in the active set approximates the best candidate in the full partition. When $\eta_i$ is close to $1$, the active set already captures the most informative candidates in partition $i$. Otherwise, when $\eta_i<\tau$, the algorithm expands $A_i$ by activating an additional element with large marginal gain (lines~10--12), provided that not all elements in $B_i$ have already been activated. In this way, new candidates are introduced only when the current active set is no longer sufficiently representative of the best elements in the partition. Given the active sets $\{A_i\}_{i=1}^N$, the ascent direction is constructed by selecting, within each partition, the active element with the largest marginal gain (lines~16--19). Formally, the direction vector $\vect{v}$ is defined by
\[
v_{(i,j_i^\star)}=1,
\qquad
j_i^\star \in \arg\max_{j\in A_i} [\nabla f(\vect{x})]_{(i,j)},
\]
and is zero otherwise. The decision vector is then updated according to the standard continuous greedy rule (line~22). After $T$ iterations, a standard rounding procedure, such as pipage rounding or swap rounding as used in the classical continuous greedy method, is applied to convert the fractional point $\vect{x}$ into a feasible set $S\in\mathcal I$ (line~24).


This thresholding mechanism naturally leads to a communication-aware variant of the continuous greedy procedure in distributed environments. In decentralized or federated implementations, each active coordinate of $\vect{x}$ corresponds to an element whose information (e.g., features or marginal gains) must be communicated across agents in order to evaluate the global objective. Rather than activating all elements in advance, \textit{ATCG} expands the active sets adaptively through the progress-ratio rule. Specifically, a new element is introduced into $A_i$ only when the current active set fails to capture a sufficiently strong marginal gain, i.e., when $\eta_i<\tau$. This mechanism avoids unnecessary activation of elements when the existing candidates already provide near-optimal marginal contributions. As a result, the number of coordinates participating in the updates and therefore the potential communication cost in distributed implementations scales with $|A_i|$ rather than the full partition size $|B_i|$.

The complete procedure of the proposed method is summarized in Algorithm~\ref{alg:atcg}. The algorithm preserves the ascent structure of the continuous greedy framework while adaptively restricting updates to a smaller set of informative candidates within each partition, thereby improving scalability without sacrificing solution quality.


%cg method below 
\begin{algorithm}[t]\footnotesize
\caption{\textbf{Continuous Greedy (CG)}}
\label{alg:cg}
\begin{algorithmic}[1]\footnotesize
\Require Ground set $\mathcal{V} = \bigcup_{i=1}^N B_i$ with disjoint partitions $B_i$; horizon $T$
\State Initialize $\vect{x} \leftarrow \vect{0}$
\For{$t = 0,1,\dots,T-1$}
    \State $\vect{v} \leftarrow \vect{0}$
    \For{$i = 1,\dots,N$}
        \State $j_i^\star \in \arg\max_{j \in B_i} [\nabla f(\vect{x})]_{(i,j)}$
        \State $v_{(i,j_i^\star)} \leftarrow 1$
    \EndFor
    \State $\vect{x} \leftarrow \vect{x} + \tfrac{1}{T}\vect{v}$
\EndFor
\State \textbf{Rounding procedure:} Round $\vect{x}$ to a feasible set $S \in \mathcal I$
\State \Return $S$
\end{algorithmic}
\end{algorithm}



% \begin{algorithm}[t]\small
% \caption{\textbf{\underline{A}daptive \underline{T}hresholded \underline{C}ontinuous \underline{G}reedy (\textit{ATCG})}}
% \label{alg:atcg}
% \label{alg:cgeta}
% \begin{algorithmic}[1]
% \Require Ground set $\mathcal{V} = \bigcup_{i=1}^N B_i$ with disjoint partitions $B_i$; active-set budgets $\rho_i$; threshold $\tau > 0$; horizon $T$; number of samples $S$
% \State Initialize $\vect{x} \leftarrow \vect{0}$
% \State Initialize active sets $A_i \leftarrow \emptyset$ for all $i = 1,\dots,N$
% \For{$t = 0,1,\dots,T-1$}
%     \State Estimate gradient $\vect{g} \approx \nabla f(\vect{x})$ using $S$ Monte Carlo samples
%     \For{$i = 1,\dots,N$}
%         \State Compute $G_i^{\max} = \max_{j \in B_i} g_{(i,j)}$
%         \If{$A_i = \emptyset$}
%             \State $\eta_i \leftarrow 0$
%         \Else
%             \State Compute $G_{i,A}^{\max} = \max_{j \in A_i} g_{(i,j)}$
%             \State $\eta_i \leftarrow \dfrac{G_{i,A}^{\max}}{G_i^{\max} + 10^{-12}}$
%         \EndIf
%         \If{$\eta_i < \tau$ and $|A_i| < \rho_i$}
%             \State $j_i^\star \in \arg\max_{j \in B_i \setminus A_i} g_{(i,j)}$
%             \State $A_i \leftarrow A_i \cup \{ j_i^\star \}$
%         \EndIf
%     \EndFor
%     \State $\vect{v} \leftarrow \vect{0}$
%     \For{$i = 1,\dots,N$}
%         \If{$A_i \neq \emptyset$}
%             \State $j_i^\star \in \arg\max_{j \in A_i} g_{(i,j)}$
%             \State $v_{(i,j_i^\star)} \leftarrow 1$
%         \EndIf
%     \EndFor
%     \State $\vect{x} \leftarrow \vect{x} + \tfrac{1}{T}\vect{v}$
% \EndFor
% % \State \textbf{Rounding:} For each partition $i$, select $b_i^\star = \arg\max_{j \in B_i} x_{(i,j)}$
% \State \textbf{Rounding procedure:} Round $\vect{x}$ to a feasible set $S \in \mathcal I$
% \State \Return $S = \{(i,b_i^\star) : i = 1,\dots,N\}$
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[t]\footnotesize
\caption{\textbf{Adaptive Thresholded Continuous Greedy (\textit{ATCG})}}
\label{alg:atcg}
\begin{algorithmic}[1]\footnotesize
\Require Ground set $\mathcal{V} = \bigcup_{i=1}^N B_i$ with disjoint partitions $B_i$; threshold $\tau > 0$; horizon $T$
\State Initialize $\vect{x} \leftarrow \vect{0}$
\State Initialize active sets $A_i \leftarrow \emptyset$ for all $i=1,\dots,N$
\For{$t = 0,1,\dots,T-1$}
    \For{$i = 1,\dots,N$}
        \If{$A_i = \emptyset$}
            \State $\eta_i \leftarrow 0$
        \Else
            \State $\eta_i \leftarrow
            \dfrac{\max_{j \in A_i} [\nabla f(\vect{x})]_{(i,j)}}
            {\max_{j \in B_i} [\nabla f(\vect{x})]_{(i,j)} + 10^{-12}}$
        \EndIf
        % \If{$\eta_i < \tau$}
        %     \State $j_i^\star \in \arg\max_{j \in B_i \setminus A_i} [\nabla f(\vect{x})]_{(i,j)}$
        %     \State $A_i \leftarrow A_i \cup \{j_i^\star\}$
        % \EndIf
        \If{$\eta_i < \tau$ and $A_i \neq B_i$}
            \State $j_i^\star \in \arg\max_{j \in B_i \setminus A_i}        [\nabla f(\vect{x})]_{(i,j)}$
         \State $A_i \leftarrow A_i \cup \{j_i^\star\}$
        \EndIf

    \EndFor
    \State $\vect{v} \leftarrow \vect{0}$
    \For{$i = 1,\dots,N$}
        \If{$A_i \neq \emptyset$}
            \State $j_i^\star \in \arg\max_{j \in A_i} [\nabla f(\vect{x})]_{(i,j)}$
            \State $v_{(i,j_i^\star)} \leftarrow 1$
        \EndIf
    \EndFor
    \State $\vect{x} \leftarrow \vect{x} + \tfrac{1}{T}\vect{v}$
\EndFor
\State \textbf{Rounding procedure:} Round $\vect{x}$ to a feasible set $S \in \mathcal I$
\State \Return $S$
\end{algorithmic}
\end{algorithm}


\subsection{Performance guarantee of \textit{ATCG} algorithm}

%new
For simplicity of analysis, we present the theoretical guarantees for the case $\kappa_i = 1$ for all partitions $i$, so that at most one element is selected from each partition. In this case, the linear maximization oracle of the continuous greedy method reduces to selecting the element with the largest gradient value in each partition. The same proof strategy extends naturally to the general case $\kappa_i > 1$ by replacing the single-element oracle and the ratio in~\eqref{eq:tau-coverage} with their top-$\kappa_i$ analogues. The next result shows that, under the $\tau$-coverage condition, \textit{ATCG} behaves as a $\tau$-approximate continuous greedy oracle. 

% Consequently, the classical $(1-e^{-1})$ approximation factor of continuous greedy degrades to $(1-e^{-\tau})$.



\begin{thm}[Performance guarantee of \textit{ATCG} algorithm \ref{alg:atcg}]
\label{thm:atcg_tau}
Consider the continuous-time version of \textit{ATCG} for a monotone submodular function $F$, and let $f$ denote its multilinear extension over the partition matroid polytope $\mathcal P$. For simplicity, assume $\kappa_i = 1$ for all partitions $i\in\{1,\dots,N\}$. By construction of \textit{ATCG}, the active-set update rule ensures that, at each iteration and for every partition $i$, the selected active set satisfies
\begin{equation}
\label{eq:tau-coverage}
\max_{j\in A_i(t)} [\nabla f(\vect{x}(t))]_{(i,j)}
\;\ge\;
\tau \max_{j\in B_i} [\nabla f(\vect{x}(t))]_{(i,j)},
\end{equation}
for some $\tau\in(0,1]$ and all $t\in[0,1]$. Let $\vect{x}^\star\in\mathcal P$ be an optimal solution of \eqref{eq::continuous}. Then the \textit{ATCG} trajectory satisfies
\[
f(\vect{x}(t)) \;\ge\; \bigl(1-e^{-\tau t}\bigr)\,f(\vect{x}^\star),
\qquad \forall t\in[0,1].
\]
In particular, at $t=1$,
\[
f(\vect{x}(1)) \;\ge\; \bigl(1-e^{-\tau}\bigr)\,f(\vect{x}^\star).
\]
\end{thm}


\begin{proof}
Let $\vect{v}_{\mathrm{ATCG}}(t)$ denote the ascent direction selected by \textit{ATCG} at time $t$, and let
\[
\bar{\vect{v}}(t)\in \arg\max_{\vect{v}\in\mathcal P}
\langle \vect{v}, \nabla f(\vect{x}(t))\rangle
\]
denote the exact continuous greedy direction.

Since $\kappa_i = 1$ for every partition, the linear maximization oracle decomposes across partitions. Hence, for each partition $i$, the exact oracle selects
\[
j_i^\star(t)\in \arg\max_{j\in B_i} [\nabla f(\vect{x}(t))]_{(i,j)},
\]
while \textit{ATCG} selects
\[
\hat{j}_i(t)\in \arg\max_{j\in A_i(t)} [\nabla f(\vect{x}(t))]_{(i,j)}.
\]
By the $\tau$-coverage condition~\eqref{eq:tau-coverage},
\[
[\nabla f(\vect{x}(t))]_{(i,\hat{j}_i(t))}
\;\ge\;
\tau\,[\nabla f(\vect{x}(t))]_{(i,j_i^\star(t))},
\qquad \forall i.
\]
Summing over all partitions yields
\[
\langle \vect{v}_{\mathrm{ATCG}}(t), \nabla f(\vect{x}(t))\rangle
\;\ge\;
\tau\,
\langle \bar{\vect{v}}(t), \nabla f(\vect{x}(t))\rangle.
\]
Since $\vect{x}^\star\in\mathcal P$, optimality of $\bar{\vect{v}}(t)$ implies
\[
\langle \bar{\vect{v}}(t), \nabla f(\vect{x}(t))\rangle
\;\ge\;
\langle \vect{x}^\star, \nabla f(\vect{x}(t))\rangle.
\]
Moreover, a standard property of the multilinear extension of a monotone submodular function states that
\[
\langle \vect{x}^\star, \nabla f(\vect{x}(t))\rangle
\;\ge\;
f(\vect{x}^\star)-f(\vect{x}(t)).
\]
Combining the previous inequalities gives
\[
\langle \vect{v}_{\mathrm{ATCG}}(t), \nabla f(\vect{x}(t))\rangle
\;\ge\;
\tau\bigl(f(\vect{x}^\star)-f(\vect{x}(t))\bigr).
\]
Since $\dot{\vect{x}}(t)=\vect{v}_{\mathrm{ATCG}}(t)$, we have by the chain rule
\[
\frac{d}{dt} f(\vect{x}(t))
=
\langle \nabla f(\vect{x}(t)), \dot{\vect{x}}(t)\rangle
=
\langle \nabla f(\vect{x}(t)), \vect{v}_{\mathrm{ATCG}}(t)\rangle.
\]
Therefore,
\[
\frac{d}{dt} f(\vect{x}(t))
\;\ge\;
\tau\bigl(f(\vect{x}^\star)-f(\vect{x}(t))\bigr).
\]
Define
\[
g(t):=f(\vect{x}^\star)-f(\vect{x}(t)).
\]
Then
\[
g'(t)\le -\tau g(t).
\]
By the comparison lemma \cite{khalil2002nonlinear}, and using $f(\vect{x}(0))=f(\vect{0})=0$, we obtain
\[
g(t)\le e^{-\tau t}g(0)=e^{-\tau t}f(\vect{x}^\star).
\]
Equivalently,
\[
f(\vect{x}(t))
\;\ge\;
\bigl(1-e^{-\tau t}\bigr)\,f(\vect{x}^\star).
\]
Setting $t=1$ completes the proof.
Consequently, similar to the classical continuous greedy method, applying a standard pipage rounding or swap rounding procedure to the fractional solution $\vect{x}(1)$ yields a feasible discrete set $S_{\textit{ATCG}} \in \mathcal I$ satisfying
\[
\mathbb{E}\big[F(S_{\textit{ATCG}})\big]
\;\ge\;
\bigl(1-e^{-\tau}\bigr)\,F(S^\star),
\qquad
S^\star \in \arg\max_{S\in\mathcal I} F(S).
\]

\end{proof}

\begin{remark}[Comparison with classical continuous greedy]
\label{rem:cg_comparison}
Theorem~\ref{thm:atcg_tau} shows that \textit{ATCG} preserves the same exponential improvement structure as classical continuous greedy, but with rate parameter $\tau$ in place of $1$. In particular, the classical continuous greedy method satisfies
$
f(\vect{x}(1)) \ge (1-e^{-1})f(\vect{x}^\star),
$
whereas \textit{ATCG} satisfies
$
f(\vect{x}(1)) \ge (1-e^{-\tau})f(\vect{x}^\star).
$
Thus, the thresholding mechanism effectively replaces the exact continuous greedy oracle with a $\tau$-approximate oracle induced by the active sets. When $\tau=1$, the bound reduces to the classical continuous greedy guarantee. More generally, as $\tau$ decreases, the convergence remains monotone but becomes more conservative, with the approximation factor degrading smoothly according to the quality of the active-set coverage. The numerical results further illustrate that the threshold parameter $\tau$ is especially beneficial in networked settings, where communication cost scales with the number of active elements. By keeping only the most informative candidates active and avoiding unnecessary additions that yield limited improvement in coverage, \textit{ATCG} significantly reduces communication overhead while preserving strong optimization performance.
\boxed{}
\end{remark}


\subsection{Curvature-aware guarantee of \textit{ATCG} algorithm}

Theorem~\ref{thm:atcg_tau} establishes a worst-case performance guarantee for \textit{ATCG} under the $\tau$-coverage condition. In particular, the resulting rate
$
1-e^{-\tau}
$
should be interpreted as a conservative baseline. In other words, it is determined entirely by the threshold parameter $\tau$ and does not exploit any additional structure of the submodular objective. In practice, however, the behavior of \textit{ATCG} can be substantially better when the objective has low total curvature.

Intuitively, low curvature means that the marginal contribution of an element does not deteriorate too much as other elements become active. In the context of \textit{ATCG}, this is especially favorable since if a partition already contains a highly informative candidate in its active set, then low curvature implies that this candidate remains competitive throughout the trajectory, even as the decision vector evolves. As a result, the active-set ratio can remain significantly larger than the nominal threshold level $\tau$, and the effective oracle quality of \textit{ATCG} becomes closer to that of the full continuous greedy method.

The next result formalizes this observation. It shows that if, in each partition, the active set contains the best singleton element, then the active-set ratio is automatically lower bounded by $1-c$, where $c$ is the total curvature of the objective. Consequently, the effective convergence rate improves from $\tau$ to $\max\{\tau,1-c\}$. In particular, as $c\to 0$, the guarantee approaches the classical continuous greedy rate.

\begin{thm}[Curvature-aware guarantee for \textit{ATCG}]
\label{cor:atcg_curvature}
Under the assumptions of Theorem~\ref{thm:atcg_tau}, let $F$ have total curvature $c\in[0,1]$. For each partition $B_i$, define
$
j_i^\circ \in \arg\max_{j\in B_i} F(\{(i,j)\}),
$
and suppose that
\[
j_i^\circ \in A_i(t), \qquad \forall i\in\{1,\dots,N\},\ \forall t\in[0,1].
\]
Then, for every partition $i$ and every $t\in[0,1]$,
\[
\max_{j\in A_i(t)} [\nabla f(\vect{x}(t))]_{(i,j)}
\;\ge\;
(1-c)\max_{j\in B_i} [\nabla f(\vect{x}(t))]_{(i,j)}.
\]
Consequently, the \textit{ATCG} trajectory satisfies
\[
f(\vect{x}(t))
\;\ge\;
\bigl(1-e^{-\max\{\tau,\,1-c\}t}\bigr)\,f(\vect{x}^\star),
\qquad \forall t\in[0,1].
\]
In particular, at $t=1$,
\[
f(\vect{x}(1))
\;\ge\;
\bigl(1-e^{-\max\{\tau,\,1-c\}}\bigr)\,f(\vect{x}^\star).
\]
\end{thm}

\begin{proof}
Fix any $t\in[0,1]$ and any partition $i$. Since $j_i^\circ \in A_i(t)$ by assumption,
\[
\max_{j\in A_i(t)} [\nabla f(\vect{x}(t))]_{(i,j)}
\;\ge\;
[\nabla f(\vect{x}(t))]_{(i,j_i^\circ)}.
\]
Now, by the curvature bound for the multilinear extension, it holds for every $(i,j)\in\mathcal V$ that \cite{vondrak1978submodularity}
\[
(1-c)\,F(\{(i,j)\})
\;\le\;
[\nabla f(\vect{x}(t))]_{(i,j)}
\;\le\;
F(\{(i,j)\}),
\]
Applying the lower bound to the singleton maximizer $j_i^\circ$ gives
\[
[\nabla f(\vect{x}(t))]_{(i,j_i^\circ)}
\;\ge\;
(1-c)\,F(\{(i,j_i^\circ)\}).
\]
On the other hand, for any $j\in B_i$,
\[
[\nabla f(\vect{x}(t))]_{(i,j)}
\;\le\;
F(\{(i,j)\}),
\]
and therefore
\[
\max_{j\in B_i} [\nabla f(\vect{x}(t))]_{(i,j)}
\;\le\;
\max_{j\in B_i} F(\{(i,j)\})
=
F(\{(i,j_i^\circ)\}).
\]
Combining the previous inequalities yields
\[
\max_{j\in A_i(t)} [\nabla f(\vect{x}(t))]_{(i,j)}
\;\ge\;
(1-c)\max_{j\in B_i} [\nabla f(\vect{x}(t))]_{(i,j)}.
\]
Since $t$ was arbitrary, this bound holds for all $t\in[0,1]$ and all partitions $i$. Thus, in addition to the threshold-based coverage level $\tau$ from Theorem~\ref{thm:atcg_tau}, the active sets also satisfy a curvature-induced coverage level of $1-c$. Hence the effective oracle quality is at least
$
\tau_{\mathrm{eff}} = \max\{\tau,1-c\}.
$
Repeating the proof of Theorem~\ref{thm:atcg_tau} with $\tau_{\mathrm{eff}}$ in place of $\tau$ gives

% \[
% \frac{d}{dt} f(\vect{x}(t))
% \;\ge\;
% \tau_{\mathrm{eff}}\bigl(f(\vect{x}^\star)-f(\vect{x}(t))\bigr).
% \]
% Defining
% \[
% g(t):=f(\vect{x}^\star)-f(\vect{x}(t)),
% \]
% we obtain
% \[
% g'(t)\le -\tau_{\mathrm{eff}}\,g(t).
% \]
% Using the comparison lemma together with $f(\vect{x}(0))=f(\vect{0})=0$, it follows that
% \[
% g(t)\le e^{-\tau_{\mathrm{eff}}t}f(\vect{x}^\star),
% \]
% which is equivalent to
\[
f(\vect{x}(t))
\;\ge\;
\bigl(1-e^{-\tau_{\mathrm{eff}}t}\bigr)\,f(\vect{x}^\star).
\]
Substituting $\tau_{\mathrm{eff}}=\max\{\tau,1-c\}$ completes the proof.
\end{proof}

\begin{remark}[Interpretation of the curvature improvement]
\label{rem:curvature_atcg}
Theorem~\ref{cor:atcg_curvature} shows that low-curvature submodular objectives are particularly favorable for \textit{ATCG}. When $c$ is small, the marginal gains of informative elements remain relatively stable as the trajectory evolves, so retaining the best singleton representative in each partition is sufficient to ensure that the active set continues to capture a large fraction of the useful marginal gains. In this regime, the effective rate parameter becomes
$
\max\{\tau,1-c\},
$ which approaches $1$ as $c\to 0$. Consequently, the guarantee of \textit{ATCG} approaches the classical continuous greedy bound
$
f(\vect{x}(1)) \ge (1-e^{-1})f(\vect{x}^\star).
$
This also explains the practical behavior observed in low-curvature problems which means a small active set can continue to capture most of the useful marginal information, thereby reducing communication overhead without substantially sacrificing optimization performance.
\end{remark}




\begin{figure}[t]
\centering
    \includegraphics[scale=0.32]{Fig/fig_atcg_rbf_heatmap.png}
\caption{\small Inter-class mean RBF similarity matrix for the CIFAR animal subset, showcasing the coupling effect between the animal images.}\vspace{-0.1in}
    \label{fig:rbf_cifar_coupling}
\end{figure}


% \begin{figure}[t]
% \centering
%     \includegraphics[scale=0.33]{Fig/tau1_trajectory.png}
% \caption{\small Facility-location objective trajectory for CG and \textit{ATCG} with $\tau=0.30$ on the CIFAR animal subset. The results show that \textit{ATCG} closely tracks the performance of CG while using a thresholded active-set update rule.}
% \label{fig:traj_cifar_atcg}
% \end{figure}



==> Algorithm_design_v1.tex <==
\section{Proposed Algorithm and Theoretical 
Guarantee}\label{sec:algo_theory}

\textit{ATCG} (Algorithm~\ref{alg:atcg}) modifies the CG 
oracle by restricting gradient evaluations to dynamically 
expanding \emph{active sets} $\{\mathcal{A}_i\}_{i=1}^N$, 
where $\mathcal{A}_i \subseteq \mathcal{P}_i$ contains the 
candidate elements of block $i$ currently participating in 
the greedy updates. Elements are admitted to $\mathcal{A}_i$ 
only when the current active set is no longer sufficiently 
representative of the best available marginal gain in 
$\mathcal{P}_i$. Since $[\mathbf{x}]_j$ can become 
non-zero only if $j \in \mathcal{A}_i$ at some iteration, 
this selective activation directly bounds which feature 
embeddings must ever be transmitted to the server.

\paragraph{Classical CG baseline.}
For completeness, we recall that CG initializes 
$\mathbf{x}(0)=\mathbf{0}$ and iterates~\eqref{eq::CG_update} 
for $T$ steps. As noted at the end of 
Section~\ref{sec::problem}, we set $\kappa_i=1$ for 
all $i\in[N]$. Under this convention, the oracle 
in~\eqref{eq::oracle_decomp} reduces to identifying, 
within each block, the single element with the largest 
gradient value:
\begin{equation*}
j_i^\star \in \operatorname*{arg\,max}_{j\in\mathcal{P}_i}
[\nabla F(\mathbf{x})]_j,
\qquad
[\mathbf{v}]_{j_i^\star} = 1,
\end{equation*}
with $[\mathbf{v}]_j=0$ otherwise and 
$\mathbf{x}\leftarrow\mathbf{x}+\tfrac{1}{T}\mathbf{v}$. 
Gradient entries are estimated via Monte Carlo 
sampling~\eqref{eq::grad}. Algorithm~\ref{alg:cg} 
gives the complete pseudocode.

\paragraph{Progress ratio.}
At each iteration, the quality of the active set 
$\mathcal{A}_i$ is measured by the \emph{progress ratio}
\begin{equation}\label{eq:eta_def}
\eta_i =
\frac{\max_{j\in\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j}
{\max_{j\in\mathcal{P}_i}
[\nabla F(\mathbf{x})]_j},
\end{equation}
the ratio of the best marginal gain within the active 
set to that of the full block $\mathcal{P}_i$. When 
$\eta_i\geq\tau$, the active set captures at least 
a $\tau$-fraction of the maximum available marginal 
gain and no expansion is needed. When $\eta_i<\tau$---
and provided $\mathcal{A}_i\neq\mathcal{P}_i$---\textit{ATCG} 
admits the element with the largest gradient value 
outside the current active set:
\begin{equation*}
j_i^\star \in 
\operatorname*{arg\,max}_{j\in\mathcal{P}_i
\setminus\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j,
\qquad
\mathcal{A}_i \leftarrow \mathcal{A}_i\cup\{j_i^\star\}.
\end{equation*}
The term ``Adaptive'' in \textit{ATCG} reflects this 
iteration-by-iteration expansion rule: the active set 
grows only when the current set is demonstrably 
insufficient, in contrast to static or pre-defined 
truncation schemes that fix participation in advance.

\paragraph{Ascent direction and update.}
Given $\{\mathcal{A}_i\}_{i=1}^N$, the ascent 
direction $\mathbf{v}$ is formed by selecting, within 
each block, the active element with the largest gradient 
value:
\begin{equation}\label{eq:atcg_dir}
j_i^\star \in \operatorname*{arg\,max}_{j\in\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j,
\qquad
[\mathbf{v}]_{j_i^\star}=1,
\end{equation}
with $[\mathbf{v}]_j=0$ otherwise. The decision 
vector is then updated as 
$\mathbf{x}\leftarrow\mathbf{x}+\tfrac{1}{T}\mathbf{v}$. 
After $T$ iterations, pipage or swap rounding converts 
the fractional solution $\mathbf{x}(1)\in\mathcal{M}$ 
into a feasible discrete set $\mathcal{S}\in\mathcal{I}$.

\paragraph{Distributed realization.}
Both CG and \textit{ATCG} admit an exact realization 
under the server-assisted protocol of 
Section~\ref{sec::problem}. At each iteration, the 
server broadcasts the block gradient 
$\{[\nabla F(\mathbf{x}(t))]_j\}_{j\in\mathcal{P}_i}$ 
to each agent $i$. For \textit{ATCG}, agent $i$ 
independently evaluates the progress 
ratio~\eqref{eq:eta_def}, performs the expansion step 
if $\eta_i < \tau$, and computes the local ascent 
direction via~\eqref{eq:atcg_dir}. Agent $i$ then 
updates its sub-vector $\mathbf{x}_i$ and uploads the 
feature embedding of any newly activated element 
$j \in \mathcal{P}_i$---i.e., any $j$ for which 
$[\mathbf{x}]_j$ transitions from zero to non-zero for 
the first time---to the server for use in subsequent 
gradient estimation. All per-block computations proceed 
in parallel, with the server serving as the sole 
coordination point.

\paragraph{Communication efficiency.}
In the server-assisted setting of 
Section~\ref{sec::problem}, only elements with 
$[\mathbf{x}]_j>0$ require their feature embeddings 
to be held at the server. Since $[\mathbf{x}]_j$ 
becomes non-zero only upon activation into $\mathcal{A}_i$, 
the total number of distinct feature embeddings ever 
uploaded is bounded by 
$\sum_{i=1}^N|\mathcal{A}_i|\ll|\mathcal{P}|$ for 
moderate $\tau$. By triggering expansion only when 
$\eta_i<\tau$, \textit{ATCG} prevents unnecessary feature 
transmissions whenever the active set already captures 
near-optimal marginal gain, keeping communication cost 
proportional to $|\mathcal{A}_i|$ rather than 
$|\mathcal{P}_i|$.


%--- CG BASELINE ALGORITHM ---%
\begin{algorithm}[t]\footnotesize
\caption{\textbf{Continuous Greedy (CG)}}
\label{alg:cg}
\begin{algorithmic}[1]\footnotesize
\Require Ground set 
$\mathcal{P}=\bigcup_{i=1}^N\mathcal{P}_i$ with 
disjoint blocks $\mathcal{P}_i$; horizon $T$; 
number of samples $K$
\State Initialize $\mathbf{x}\leftarrow\mathbf{0}$
\For{$t=0,1,\ldots,T-1$}
    \State Estimate gradient 
    $\mathbf{g}\approx\nabla F(\mathbf{x})$ 
    using $K$ Monte Carlo samples 
    via~\eqref{eq::grad}
    \State Set $\mathbf{v}\leftarrow\mathbf{0}$
    \For{$i=1,\ldots,N$}
        \State $j_i^\star\in
        \operatorname*{arg\,max}_{j\in\mathcal{P}_i}
        [\mathbf{g}]_j$
        \State $[\mathbf{v}]_{j_i^\star}
        \leftarrow 1$
    \EndFor
    \State $\mathbf{x}\leftarrow
    \mathbf{x}+\tfrac{1}{T}\mathbf{v}$
\EndFor
\State \textbf{Rounding:} Round $\mathbf{x}$ to a 
feasible set $\mathcal{S}\in\mathcal{I}$
\State \Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


%--- ATCG ALGORITHM ---%
\begin{algorithm}[t]\footnotesize
\caption{\textbf{Adaptive Thresholded Continuous 
Greedy (\textit{ATCG})}}
\label{alg:atcg}
\begin{algorithmic}[1]\footnotesize
\Require Ground set 
$\mathcal{P}=\bigcup_{i=1}^N\mathcal{P}_i$ with 
disjoint blocks $\mathcal{P}_i$; threshold $\tau>0$; 
horizon $T$; number of samples $K$
\State Initialize $\mathbf{x}\leftarrow\mathbf{0}$
\State Initialize active sets 
$\mathcal{A}_i\leftarrow\emptyset$ for all 
$i=1,\ldots,N$
\For{$t=0,1,\ldots,T-1$}
    \State Estimate gradient 
    $\mathbf{g}\approx\nabla F(\mathbf{x})$ 
    using $K$ Monte Carlo samples 
    via~\eqref{eq::grad}
    \For{$i=1,\ldots,N$} 
    \hfill$\triangleright$ \textit{Progress check 
    and expansion}
        \If{$\mathcal{A}_i=\emptyset$}
            \State $\eta_i\leftarrow 0$
        \Else
            \State $\eta_i\leftarrow
            \dfrac{\max_{j\in\mathcal{A}_i}
            [\mathbf{g}]_j}
            {\max_{j\in\mathcal{P}_i}
            [\mathbf{g}]_j+10^{-12}}$
        \EndIf
        \If{$\eta_i<\tau$ \textbf{and} 
        $\mathcal{A}_i\neq\mathcal{P}_i$}
            \State $j_i^\star\in
            \operatorname*{arg\,max}_{j\in
            \mathcal{P}_i\setminus\mathcal{A}_i}
            [\mathbf{g}]_j$
            \State $\mathcal{A}_i\leftarrow
            \mathcal{A}_i\cup\{j_i^\star\}$
        \EndIf
    \EndFor
    \State Set $\mathbf{v}\leftarrow\mathbf{0}$
    \For{$i=1,\ldots,N$} 
    \hfill$\triangleright$ \textit{Active-set oracle}
        \If{$\mathcal{A}_i\neq\emptyset$}
            \State $j_i^\star\in
            \operatorname*{arg\,max}_{j\in\mathcal{A}_i}
            [\mathbf{g}]_j$
            \State $[\mathbf{v}]_{j_i^\star}
            \leftarrow 1$
        \EndIf
    \EndFor
    \State $\mathbf{x}\leftarrow
    \mathbf{x}+\tfrac{1}{T}\mathbf{v}$
\EndFor
\State \textbf{Rounding:} Round $\mathbf{x}$ to a 
feasible set $\mathcal{S}\in\mathcal{I}$
\State \Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

\subsection{Performance Guarantee of \textit{ATCG}}

For simplicity of analysis, we present the theoretical guarantees 
for the case $\kappa_i = 1$ for all $i\in\{1,\dots,N\}$, so that 
at most one element is selected from each block. In this case, the 
linear maximization oracle reduces to selecting the element with the 
largest gradient value in each block $\mathcal{P}_i$. The same proof 
strategy extends naturally to the general case $\kappa_i > 1$ by 
replacing the single-element oracle and the ratio 
in~\eqref{eq:eta_def} with their top-$\kappa_i$ analogues. The 
next result shows that, under the $\tau$-coverage condition, 
\textit{ATCG} behaves as a $\tau$-approximate continuous greedy 
oracle.

\begin{thm}[Performance guarantee of \textit{ATCG}, 
Algorithm~\ref{alg:atcg}]
\label{thm:atcg_tau}
Consider the continuous-time version of \textit{ATCG} for a monotone 
submodular function $f:2^{\mathcal{P}}\to\mathbb{R}_{+}$, and let 
$F$ denote its multilinear extension over the matroid polytope 
$\mathcal{M}$. Assume $\kappa_i = 1$ for all $i\in\{1,\dots,N\}$. 
By construction of \textit{ATCG}, the active-set update rule ensures 
that, at each iteration and for every block $i$, the selected active 
set satisfies the $\tau$-coverage condition:
\begin{equation}\label{eq:tau-coverage}
\max_{j\in\mathcal{A}_i(t)} [\nabla F(\mathbf{x}(t))]_j
\;\geq\;
\tau \max_{j\in\mathcal{P}_i} [\nabla F(\mathbf{x}(t))]_j,
\end{equation}
for some $\tau\in(0,1]$ and all $t\in[0,1]$. Let 
$\mathbf{x}^\star\in\mathcal{M}$ be an optimal solution 
of~\eqref{eq::cont}. Then the \textit{ATCG} trajectory satisfies
\[
F(\mathbf{x}(t)) \;\geq\; 
\bigl(1-e^{-\tau t}\bigr)\,F(\mathbf{x}^\star),
\qquad \forall\, t\in[0,1].
\]
In particular, at $t=1$,
\[
F(\mathbf{x}(1)) \;\geq\; 
\bigl(1-e^{-\tau}\bigr)\,F(\mathbf{x}^\star).
\]
\end{thm}

\begin{proof}
Let $\mathbf{v}_{\mathrm{ATCG}}(t)$ denote the ascent direction 
selected by \textit{ATCG} at time $t$, and let
\[
\bar{\mathbf{v}}(t)\in \operatorname*{arg\,max}_{\mathbf{v}
\in\mathcal{M}}\;
\mathbf{v}^{\!\top}\nabla F(\mathbf{x}(t))
\]
denote the exact continuous greedy direction. Since $\kappa_i = 1$ 
for every block, the oracle decomposes blockwise 
via~\eqref{eq::oracle_decomp}. For each block $i$, the exact oracle 
selects
\[
j_i^\star(t)\in \operatorname*{arg\,max}_{j\in\mathcal{P}_i} 
[\nabla F(\mathbf{x}(t))]_j,
\]
while \textit{ATCG} selects
\[
\hat{j}_i(t)\in \operatorname*{arg\,max}_{j\in\mathcal{A}_i(t)} 
[\nabla F(\mathbf{x}(t))]_j.
\]
By the $\tau$-coverage condition~\eqref{eq:tau-coverage},
\[
[\nabla F(\mathbf{x}(t))]_{\hat{j}_i(t)}
\;\geq\;
\tau\,[\nabla F(\mathbf{x}(t))]_{j_i^\star(t)},
\qquad \forall\, i.
\]
Summing over all blocks yields
\[
\mathbf{v}_{\mathrm{ATCG}}^{\!\top}(t)\,\nabla F(\mathbf{x}(t))
\;\geq\;
\tau\;
\bar{\mathbf{v}}^{\!\top}(t)\,\nabla F(\mathbf{x}(t)).
\]
Since $\mathbf{x}^\star\in\mathcal{M}$, optimality of 
$\bar{\mathbf{v}}(t)$ gives
\[
\bar{\mathbf{v}}^{\!\top}(t)\,\nabla F(\mathbf{x}(t))
\;\geq\;
{\mathbf{x}^\star}^{\!\top}\nabla F(\mathbf{x}(t)).
\]
Moreover, a standard property of the multilinear extension of a 
monotone submodular function states that
\[
{\mathbf{x}^\star}^{\!\top}\nabla F(\mathbf{x}(t))
\;\geq\;
F(\mathbf{x}^\star)-F(\mathbf{x}(t)).
\]
Combining the three inequalities gives
\[
\mathbf{v}_{\mathrm{ATCG}}^{\!\top}(t)\,\nabla F(\mathbf{x}(t))
\;\geq\;
\tau\bigl(F(\mathbf{x}^\star)-F(\mathbf{x}(t))\bigr).
\]
Since $\dot{\mathbf{x}}(t)=\mathbf{v}_{\mathrm{ATCG}}(t)$, the 
chain rule gives
\[
\frac{d}{dt} F(\mathbf{x}(t))
=
\nabla F(\mathbf{x}(t))^{\!\top}\dot{\mathbf{x}}(t)
=
\nabla F(\mathbf{x}(t))^{\!\top}\mathbf{v}_{\mathrm{ATCG}}(t).
\]
Therefore,
\[
\frac{d}{dt} F(\mathbf{x}(t))
\;\geq\;
\tau\bigl(F(\mathbf{x}^\star)-F(\mathbf{x}(t))\bigr).
\]
Define $g(t):=F(\mathbf{x}^\star)-F(\mathbf{x}(t))\geq 0$. 
Then $g'(t)\leq -\tau g(t)$. By Gr\"{o}nwall's 
inequality~\cite{khalil2002nonlinear}, and using 
$F(\mathbf{x}(0))=F(\mathbf{0})=0$,
\[
g(t)\leq e^{-\tau t}g(0)=e^{-\tau t}F(\mathbf{x}^\star).
\]
Equivalently,
\[
F(\mathbf{x}(t))
\;\geq\;
\bigl(1-e^{-\tau t}\bigr)\,F(\mathbf{x}^\star).
\]
Setting $t=1$ completes the proof. Applying pipage or swap rounding 
to the fractional solution $\mathbf{x}(1)$ then yields a feasible 
discrete set $\mathcal{S}_{\textit{ATCG}}\in\mathcal{I}$ satisfying
\[
\mathbb{E}\bigl[f(\mathcal{S}_{\textit{ATCG}})\bigr]
\;\geq\;
\bigl(1-e^{-\tau}\bigr)\,f(\mathcal{S}^\star),
\qquad
\mathcal{S}^\star \in 
\operatorname*{arg\,max}_{\mathcal{S}\in\mathcal{I}} f(\mathcal{S}).
\]
\end{proof}

\begin{remark}[Comparison with classical continuous greedy]
\label{rem:cg_comparison}
Theorem~\ref{thm:atcg_tau} shows that \textit{ATCG} preserves the 
same exponential improvement structure as classical continuous greedy, 
but with rate parameter $\tau$ in place of $1$. In particular, 
classical CG satisfies 
$F(\mathbf{x}(1)) \geq (1-e^{-1})F(\mathbf{x}^\star)$,
whereas \textit{ATCG} satisfies
$F(\mathbf{x}(1)) \geq (1-e^{-\tau})F(\mathbf{x}^\star)$.
Thus, the thresholding mechanism effectively replaces the exact CG 
oracle with a $\tau$-approximate oracle induced by the active sets 
$\{\mathcal{A}_i\}$. When $\tau=1$, the bound recovers the classical 
guarantee. As $\tau$ decreases, the approximation factor degrades 
smoothly according to the active-set coverage quality, while the 
monotone ascent structure is preserved throughout. The numerical 
results further illustrate that $\tau$ is especially beneficial in 
server-assisted settings, where communication cost scales with 
$\sum_i|\mathcal{A}_i|$. By triggering expansion only when 
$\eta_i < \tau$~\eqref{eq:eta_def} and keeping only the most 
informative candidates active, \textit{ATCG} significantly reduces 
communication overhead while preserving strong optimization 
performance.
\end{remark}
\subsection{Curvature-Aware Guarantee of \textit{ATCG}}

Theorem~\ref{thm:atcg_tau} establishes a worst-case performance 
guarantee for \textit{ATCG} under the $\tau$-coverage 
condition~\eqref{eq:tau-coverage}. The resulting rate $1-e^{-\tau}$ 
is a conservative baseline, determined entirely by the threshold 
parameter $\tau$ and independent of any structural properties of the 
submodular objective. In practice, however, when $f$ has low total 
curvature, the performance of \textit{ATCG} can be substantially 
stronger.

Intuitively, low curvature means that the marginal contribution of an 
element does not deteriorate significantly as other elements become 
active. In the context of \textit{ATCG}, this is especially 
favorable: if block $\mathcal{P}_i$ already contains a highly 
informative candidate in its active set $\mathcal{A}_i$, low 
curvature implies that this candidate remains competitive throughout 
the trajectory, even as $\mathbf{x}$ evolves. As a result, the 
progress ratio $\eta_i$~\eqref{eq:eta_def} can remain well above the 
nominal threshold $\tau$, and the effective oracle quality of 
\textit{ATCG} approaches that of the full continuous greedy method.

The next result formalizes this observation. It shows that if, in 
each block, the active set contains the best singleton element, then 
$\eta_i$ is automatically lower-bounded by $1-c$, where $c$ is the 
total curvature of $f$. Consequently, the effective convergence rate 
improves from $\tau$ to $\max\{\tau, 1-c\}$. In particular, as 
$c\to 0$, the guarantee approaches the classical continuous greedy 
rate.

\begin{thm}[Curvature-aware guarantee for \textit{ATCG}]
\label{cor:atcg_curvature}
Under the assumptions of Theorem~\ref{thm:atcg_tau}, let $f$ have 
total curvature $c\in[0,1]$. For each block $\mathcal{P}_i$, define
\[
j_i^\circ \in \operatorname*{arg\,max}_{j\in\mathcal{P}_i}
f(\{j\}),
\]
and suppose that
\[
j_i^\circ \in \mathcal{A}_i(t),
\qquad
\forall\,i\in\{1,\ldots,N\},\;\forall\,t\in[0,1].
\]
Then, for every block $i$ and every $t\in[0,1]$,
\[
\max_{j\in\mathcal{A}_i(t)}[\nabla F(\mathbf{x}(t))]_j
\;\geq\;
(1-c)\max_{j\in\mathcal{P}_i}[\nabla F(\mathbf{x}(t))]_j.
\]
Consequently, the \textit{ATCG} trajectory satisfies
\[
F(\mathbf{x}(t))
\;\geq\;
\bigl(1-e^{-\max\{\tau,\,1-c\}\,t}\bigr)\,F(\mathbf{x}^\star),
\qquad \forall\,t\in[0,1].
\]
In particular, at $t=1$,
\[
F(\mathbf{x}(1))
\;\geq\;
\bigl(1-e^{-\max\{\tau,\,1-c\}}\bigr)\,F(\mathbf{x}^\star).
\]
\end{thm}

\begin{proof}
Fix any $t\in[0,1]$ and any block $i$. Since 
$j_i^\circ\in\mathcal{A}_i(t)$ by assumption,
\[
\max_{j\in\mathcal{A}_i(t)}[\nabla F(\mathbf{x}(t))]_j
\;\geq\;
[\nabla F(\mathbf{x}(t))]_{j_i^\circ}.
\]
By the curvature bound for the multilinear extension, for every 
$j\in\mathcal{P}$~\cite{vondrak1978submodularity},
\[
(1-c)\,f(\{j\})
\;\leq\;
[\nabla F(\mathbf{x}(t))]_j
\;\leq\;
f(\{j\}).
\]
Applying the lower bound to $j_i^\circ$ gives
\[
[\nabla F(\mathbf{x}(t))]_{j_i^\circ}
\;\geq\;
(1-c)\,f(\{j_i^\circ\}).
\]
On the other hand, the upper bound applied to any $j\in\mathcal{P}_i$ 
yields
\[
\max_{j\in\mathcal{P}_i}[\nabla F(\mathbf{x}(t))]_j
\;\leq\;
\max_{j\in\mathcal{P}_i} f(\{j\})
=
f(\{j_i^\circ\}).
\]
Combining these three inequalities,
\[
\max_{j\in\mathcal{A}_i(t)}[\nabla F(\mathbf{x}(t))]_j
\;\geq\;
(1-c)\max_{j\in\mathcal{P}_i}[\nabla F(\mathbf{x}(t))]_j.
\]
Since $t$ and $i$ were arbitrary, this bound holds for all 
$t\in[0,1]$ and all blocks $i$. Thus, in addition to the 
threshold-based coverage level $\tau$ from 
Theorem~\ref{thm:atcg_tau}, the active sets also satisfy a 
curvature-induced coverage level of $1-c$. The effective oracle 
quality is therefore at least
\[
\tau_{\mathrm{eff}} = \max\{\tau,\,1-c\}.
\]
Repeating the proof of Theorem~\ref{thm:atcg_tau} with 
$\tau_{\mathrm{eff}}$ in place of $\tau$ gives
\[
F(\mathbf{x}(t))
\;\geq\;
\bigl(1-e^{-\tau_{\mathrm{eff}}\,t}\bigr)\,F(\mathbf{x}^\star).
\]
Substituting $\tau_{\mathrm{eff}}=\max\{\tau,\,1-c\}$ completes 
the proof.
\end{proof}

\begin{remark}[Interpretation of the curvature improvement]
\label{rem:curvature_atcg}
Theorem~\ref{cor:atcg_curvature} shows that low-curvature submodular 
objectives are particularly favorable for \textit{ATCG}. When $c$ is 
small, the marginal gains of informative elements remain relatively 
stable as the trajectory evolves, so retaining the best singleton 
representative $j_i^\circ$ in each block is sufficient to ensure that 
$\mathcal{A}_i$ continues to capture a large fraction of the available 
marginal gains. In this regime, the effective rate parameter 
$\max\{\tau, 1-c\}$ approaches $1$ as $c\to 0$, and the guarantee of 
\textit{ATCG} approaches the classical continuous greedy bound 
$F(\mathbf{x}(1))\geq(1-e^{-1})F(\mathbf{x}^\star)$. In the 
server-assisted setting of Section~\ref{sec::problem}, this 
translates directly to communication efficiency: when curvature is 
low, a small active set $\mathcal{A}_i\subseteq\mathcal{P}_i$ 
captures near-optimal marginal information throughout the 
optimization, limiting the number of feature embeddings that must 
ever be transmitted to the server without sacrificing solution 
quality.
\end{remark}

==> Algorithm_design_v2.tex <==
\section{Proposed Algorithm and Theoretical 
Guarantees}\label{sec:algo_theory}


\textit{ATCG} (Alg.~\ref{alg:atcg}) restricts gradient evaluations to dynamically 
expanding \emph{active sets} $\mathcal{A}_i \subseteq \mathcal{P}_i$. Elements 
are admitted to $\mathcal{A}_i$ only when the current set fails to capture 
sufficient marginal gain from $\mathcal{P}_i$. Since $[\mathbf{x}]_j > 0$ 
only if $j \in \cup \mathcal{A}_i$, this selective activation bounds the 
number of feature embeddings transmitted to the server.


\paragraph{Progress ratio.}
The quality of active set $\mathcal{A}_i$ is monitored via the \emph{progress ratio} 
\begin{equation}\label{eq:eta_def}
\eta_i =
\frac{\max_{j\in\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j}
{\max_{j\in\mathcal{P}_i}
[\nabla F(\mathbf{x})]_j},
\end{equation}
If $\eta_i < \tau$ and $\mathcal{A}_i \neq \mathcal{P}_i$, the active set is expanded:
\begin{equation*}
j_i^\star \in \operatorname*{arg\,max}_{j\in\mathcal{P}_i\setminus\mathcal{A}_i} [\nabla F(\mathbf{x})]_j, \quad \mathcal{A}_i \leftarrow \mathcal{A}_i \cup \{j_i^\star\}.
\end{equation*}
Unlike static truncation schemes, \textit{ATCG} is ``adaptive'' in that $\mathcal{A}_i$ grows only when the current set fails to capture a $\tau$-fraction of the maximum available marginal gain.
\begin{comment}
\paragraph{Progress ratio.}
At each iteration, the quality of the active set 
$\mathcal{A}_i$ is measured by the \emph{progress ratio}
\begin{equation}\label{eq:eta_def}
\eta_i =
\frac{\max_{j\in\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j}
{\max_{j\in\mathcal{P}_i}
[\nabla F(\mathbf{x})]_j},
\end{equation}
the ratio of the best marginal gain within the active 
set to that of the full partition $\mathcal{P}_i$. When 
$\eta_i\geq\tau$, the active set captures at least 
a $\tau$-fraction of the maximum available marginal 
gain and no expansion is needed. When $\eta_i<\tau$ 
and provided $\mathcal{A}_i\neq\mathcal{P}_i$, \textit{ATCG} 
admits the element with the largest gradient value 
outside the current active set:
\begin{equation*}
j_i^\star \in 
\operatorname*{arg\,max}_{j\in\mathcal{P}_i
\setminus\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j,
\qquad
\mathcal{A}_i \leftarrow \mathcal{A}_i\cup\{j_i^\star\}.
\end{equation*}
The term ``Adaptive'' in \textit{ATCG} reflects this 
iteration-by-iteration expansion rule: the active set 
grows only when the current set is demonstrably 
insufficient, in contrast to static or pre-defined 
truncation schemes that fix participation in advance.
\end{comment}
\paragraph{Ascent direction and update}
Given $\{\mathcal{A}_i\}_{i=1}^N$, \textit{ATCG} 
restricts the oracle~\eqref{eq::oracle_decomp} to the 
active set, selecting within each partition the active 
element with the largest gradient value:
\begin{equation}\label{eq:atcg_dir}
j_i^\star \in \operatorname*{arg\,max}_{j\in\mathcal{A}_i}
[\nabla F(\mathbf{x})]_j,
\qquad
[\mathbf{v}]_{j_i^\star}=1,
\end{equation}
with $[\mathbf{v}]_j=0$ otherwise, and the decision 
vector updated as 
$\mathbf{x}\leftarrow\mathbf{x}+\tfrac{1}{T}\mathbf{v}$. 
After $T$ iterations, pipage or swap rounding converts 
the fractional solution $\mathbf{x}(1)\in\mathcal{M}$ 
into a feasible discrete set $\mathcal{S}\in\mathcal{I}$.
\begin{comment}
\paragraph{Distributed realization.}
\textit{ATCG} (Alg.~\ref{alg:atcg}) is implemented via the server-assisted protocol of Section~\ref{sec::problem}. Upon receiving the global state $\mathbf{x}$ and current embedding set $\mathcal{E}$, each agent $i$ independently computes its local partition gradient $\{[\mathbf{g}]_j\}_{j\in\mathcal{P}_i}$ via~\eqref{eq::grad}. If the progress ratio $\eta_i < \tau$, agent $i$ expands $\mathcal{A}_i$ by admitting the steepest inactive gradient. Crucially, an element's feature embedding is transmitted to the server only upon its admission to $\mathcal{A}_i$, which is the necessary condition for its coordinate in $\mathbf{x}_i$ to become non-zero. Each agent then updates its sub-vector $\mathbf{x}_i$ via the local ascent direction~\eqref{eq:atcg_dir} and uploads it. All computations proceed in parallel, with the server acting as the central coordination point.
\end{comment}
\paragraph{Distributed realization}
\textit{ATCG} admits an exact realization under the 
server-assisted protocol of Section~\ref{sec::problem}, 
formalized in Algorithm~\ref{alg:atcg}. At each 
iteration, upon receiving the global state $\mathbf{x}$ 
and the current embedding set $\mathcal{E}$ from the server, 
each agent $i$ independently estimates its local partition 
gradient $\{[\mathbf{g}]_j\}_{j\in\mathcal{P}_i}$ 
via~\eqref{eq::grad}. The agent then evaluates 
the progress ratio~\eqref{eq:eta_def} and, if 
$\eta_i < \tau$, expands its active set $\mathcal{A}_i$ 
by adding the best inactive element. Crucially, the 
feature embedding of this new element is transmitted to 
the server only upon its initial entry into $\mathcal{A}_i$, 
marking the first time its corresponding coordinate in 
$\mathbf{x}_i$ can become non-zero. Agent $i$ then 
computes its local ascent direction via~\eqref{eq:atcg_dir}, 
updates its sub-vector $\mathbf{x}_i$, and uploads it to the 
server. All per-partition computations proceed in 
parallel, with the server as the sole 
coordination and assembly~point.
\begin{comment}
{\color{blue}
\paragraph{Communication saving.} In \textit{ATCG}, a feature embedding is transmitted only when
its element first enters an active set, so communication is
governed by the growth of $\{\mathcal{A}_i\}_{i=1}^N$.
Since active sets are monotone increasing and at most one
element is added per partition per iteration,
$|\mathcal{A}_i(T)|\le\min\{T,|\mathcal{P}_i|\}$, giving
$N \le C_{\mathrm{ATCG}}(T) \le |\mathcal{P}|$,
where $C_{\mathrm{ATCG}}(T)=\sum_{i=1}^{N}|\mathcal{A}_i(T)|$.
Standard \textit{CG} can select a new element per partition
at every iteration as $\mathbf{x}$ evolves, so
$C_{\mathrm{CG}}(T)\to|\mathcal{P}|$ as $T\to\infty$.
\textit{ATCG} prevents this through its per-partition threshold
mechanism: the expansion step fires only when $\eta_i(t)<\tau$,
directly gating which embeddings are ever transmitted.
The \textit{total curvature}
$c = 1 - \min_{\mathcal{S},\,p}
\frac{f(\mathcal{S}\cup\{p\})-f(\mathcal{S})}{f(\{p\})}$
measures marginal-gain deterioration as elements become
active~\cite{vondrak1978submodularity}; under low curvature
a highly informative element in $\mathcal{A}_i$ remains
competitive as $\mathbf{x}$ evolves, as formalized below.
}
\end{comment}

%--- ATCG ALGORITHM ---%
%--- SERVER-ASSISTED ATCG ALGORITHM ---%
\begin{algorithm}[t]\footnotesize
\caption{\textbf{\textit{ATCG}} in Server-Assisted Realization}
\label{alg:atcg}
\begin{algorithmic}[1]\footnotesize
\Require Ground set $\mathcal{P}=\bigcup_{i=1}^N\mathcal{P}_i$
with disjoint partitions $\mathcal{P}_i$; threshold $\tau>0$;
horizon $T$; number of MC samples $K$
\State \textbf{[Server]}\;
$\mathbf{x}\leftarrow\mathbf{0}$;\;
$\mathcal{E}\leftarrow\emptyset$
\State \textbf{[Agent $i$, $\forall i$]}\;
$\mathbf{x}_i\leftarrow\mathbf{0}$;\;
$\mathcal{A}_i\leftarrow\emptyset$
\For{$t=0,1,\ldots,T-1$}
    \State \textbf{[Server$\,\to\,$Agent $i$]}\;
    Broadcast $\mathcal{E}$ and $\mathbf{x}$ to each agent
    \hfill$\triangleright$ \textit{Incremental broadcast}
    \For{$i=1,\ldots,N$}
    \hfill$\triangleright$ \textit{Local computation (parallel)}
        \State \textbf{[Agent $i$]}\;
        Estimate $[\mathbf{g}]_j \approx [\nabla F(\mathbf{x})]_j$
        for all $j\in\mathcal{P}_i$ using $K$ MC samples
        via~\eqref{eq::grad} over $\mathcal{E}$
        \hfill$\triangleright$ \textit{Gradient estimation}
        \State \textbf{[Agent $i$]}\;
        $\eta_i \leftarrow 0$ if $\mathcal{A}_i=\emptyset$,\;
        else\;
        $\eta_i\leftarrow
        \dfrac{\max_{j\in\mathcal{A}_i}[\mathbf{g}]_j}
        {\max_{j\in\mathcal{P}_i}[\mathbf{g}]_j+10^{-12}}$
        \hfill$\triangleright$ \textit{Progress ratio}~\eqref{eq:eta_def}
        \If{$\eta_i < \tau$ \textbf{and}
        $\mathcal{A}_i \neq \mathcal{P}_i$}
        \hfill$\triangleright$ \textit{Active-set expansion}
            \State \textbf{[Agent $i$]}\;
            $j_i^\star \leftarrow
            \operatorname*{arg\,max}_{j\in
            \mathcal{P}_i\setminus\mathcal{A}_i}
            [\mathbf{g}]_j$;\;
            $\mathcal{A}_i \leftarrow
            \mathcal{A}_i \cup \{j_i^\star\}$
            \State \textbf{[Agent $i\,\to\,$Server]}\;
            Transmit embedding of $j_i^\star$;\;
            $\mathcal{E}\leftarrow\mathcal{E}
            \cup\{j_i^\star\}$
            \hfill$\triangleright$ \textit{Embedding upload}
        \EndIf
        \If{$\mathcal{A}_i \neq \emptyset$}
        \hfill$\triangleright$ \textit{Active-set oracle}~\eqref{eq:atcg_dir}
            \State \textbf{[Agent $i$]}\;
            $j_i^\star \leftarrow
            \operatorname*{arg\,max}_{j\in\mathcal{A}_i}
            [\mathbf{g}]_j$
            \State \textbf{[Agent $i$]}\;
            $[\mathbf{x}_i]_{j_i^\star} \leftarrow
            [\mathbf{x}_i]_{j_i^\star} + \tfrac{1}{T}$
        \EndIf
    \EndFor
    \For{$i=1,\ldots,N$}
    \hfill$\triangleright$ \textit{Upload (parallel)}
        \State \textbf{[Agent $i\,\to\,$Server]}\;
        Transmit $\mathbf{x}_i\!\left(t+\tfrac{1}{T}\right)$
    \EndFor
    \State \textbf{[Server]}\; Assemble
    $\mathbf{x}\!\left(t+\tfrac{1}{T}\right)=
    [\mathbf{x}_1^\top,\ldots,\mathbf{x}_N^\top]^\top$
\EndFor
\State \textbf{[Server]}\;
\textbf{Round} $\mathbf{x}(1)$ to feasible $\mathcal{S}\in\mathcal{I}$
\State \Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


%The next result shows that, under the $\tau$-coverage condition~\eqref{eq:tau-coverage}, \textit{ATCG} behaves as a $\tau$-approximate CG oracle.

% \begin{assump}[Exact-gradient and continuous-time idealization]
% \label{rem:exact_grad}
% The guarantees below are stated for the exact gradient
% $\nabla F(\mathbf{x})$ and the continuous-time ascent
% flow~\eqref{eq::CG_update} where $\vect{v}(t)$ is decided by \textit{ATCG} via~\eqref{eq:atcg_dir}. The impact of the practical
% discretization~\eqref{eq::CG_disc} and Monte Carlo
% approximation~\eqref{eq::grad} on the optimality gap follows
% the standard analysis of~\cite{calinescu2011maximizing} and
% is omitted to avoid unnecessary complexity.\boxend
% \end{assump}


\subsection{Performance Guarantee of \textit{ATCG}}

\begin{assump}[Exact-gradient and continuous-time idealization]
\label{rem:exact_grad}
The guarantees below are stated for the exact gradient
$\nabla F(\mathbf{x})$ and the continuous-time ascent
flow~\eqref{eq::CG_update} where $\vect{v}(t)$ is decided
by \textit{ATCG} via~\eqref{eq:atcg_dir}.\hfill$\square$
\end{assump}

{\color{blue}The impact of the practical discretization~\eqref{eq::CG_disc}
and Monte Carlo approximation~\eqref{eq::grad} follows the
standard analysis of~\cite{calinescu2011maximizing} and is
omitted; the finite-step error vanishes at $\mathcal{O}(1/T)$
and the gradient-estimation error decays at
$\mathcal{O}(1/\sqrt{K})$.}

\begin{thm}[Curvature-Aware Approximation Guarantee]
\label{thm:atcg_curvature}
\reza{Let Assumption~\ref{rem:exact_grad} hold. Suppose $f$ in~\eqref{eq::canonical_prob} is a monotone submodular function with total curvature $c \in [0,1]$, $F$ is its multilinear extension~\eqref{eq::multi_linear}, and $\mathcal{M}$ is the matroid polytope~\eqref{eq::polytope}. Let $\mathbf{x}^\star \in \operatorname*{arg\,max}_{\mathbf{x} \in \mathcal{M}} F(\mathbf{x})$. If $\mathbf{x}(t)$ is the solution trajectory generated by \textit{ATCG} with a threshold $\tau \in (0,1]$, then for all $t \in [0,1]$ and all partitions $i \in [N]$, the active set satisfies the effective oracle bound:}
\begin{equation}
\label{eq:effective_oracle}
\max_{j \in \mathcal{A}_i(t)} [\nabla F(\mathbf{x}(t))]_j \geq \max\{\tau, 1-c\} \max_{j \in \mathcal{P}_i} [\nabla F(\mathbf{x}(t))]_j.
\end{equation}
Consequently, the objective value satisfies:
\begin{equation}
\label{eq:convergence_guarantee}
F(\mathbf{x}(t)) \geq \left(1 - e^{-\max\{\tau, 1-c\}\,t}\right) F(\mathbf{x}^\star).
\end{equation}
In particular, the final solution at $t=1$ guarantees $F(\mathbf{x}(1)) \geq \left(1 - e^{-\max\{\tau, 1-c\}}\right) F(\mathbf{x}^\star)$.
\end{thm}





\begin{comment}
\begin{thm}[Curvature-aware guarantee for \textit{ATCG}]
\label{cor:atcg_curvature}
Let Assumption~\ref{rem:exact_grad} hold, let $f$
in~\eqref{eq::canonical_prob} be monotone submodular with
total curvature $c\in[0,1]$, let $F$ be its multilinear
extension~\eqref{eq::multi_linear}, and let $\mathcal{M}$
be the matroid polytope~\eqref{eq::polytope}.
For each partition $\mathcal{P}_i$, let
$j_i^\circ\in\arg\max_{j\in\mathcal{P}_i}f(\{j\})$.
Since $\mathbf{x}(0)=\mathbf{0}$, the initial activation
step selects $j_i^\circ$ in each partition, and by
monotonicity of the active sets,
$j_i^\circ\in\mathcal{A}_i(t)$ for all $i\in[N]$ and
$t\in[0,1]$. Then, for every partition $i$ and
$t\in[0,1]$,
\[
\max_{j\in\mathcal{A}_i(t)}[\nabla F(\mathbf{x}(t))]_j
\;\geq\;
(1-c)\max_{j\in\mathcal{P}_i}[\nabla F(\mathbf{x}(t))]_j.
\]
Therefore, $$\max_{j\in\mathcal{A}_i(t)} [\nabla F(\mathbf{x}(t))]_j
\;\geq\;
\tau \max_{j\in\mathcal{P}_i} [\nabla F(\mathbf{x}(t))]_j$$
holds with effective rate
$\tau_{\mathrm{eff}}=\max\{\tau,1-c\}$.
Letting $\mathbf{x}^\star\in\mathcal{M}$ be optimal
in~\eqref{eq::cont},
\[
F(\mathbf{x}(t))
\;\geq\;
\bigl(1-e^{-\max\{\tau,\,1-c\}\,t}\bigr)\,F(\mathbf{x}^\star),
\quad\forall\,t\in[0,1].
\]
In particular, at $t=1$,
$F(\mathbf{x}(1))\ge
\bigl(1-e^{-\max\{\tau,1-c\}}\bigr)F(\mathbf{x}^\star).$
\end{thm}
\end{comment}
Due to space limitation, the proof is given
in~\cite{rostami2026atcg}.
\begin{rem}[Special cases and Pareto structure]\label{rem:pareto}
When $c=0$, $\max\{\tau,1-c\}=1$ and the bound recovers
the classical CG rate $1-1/e$, regardless of $\tau$.
When $\tau=1-c$, the rate is $1-e^{-(1-c)}$.
For $\tau\le 1-c$, the effective rate $1-c$ is independent
of $\tau$; any $\tau<1-c$ achieves identical performance,
making such choices dominated. Increasing $\tau$ above
$1-c$ improves the approximation toward $1-1/e$ as
$\tau\to 1$, but increases communication as shown in
Section~\ref{sec::com_eff}. Hence
$\tau^\star=1-c$ is the \textit{Pareto-optimal threshold},
simultaneously attaining minimum communication and the best
approximation factor at that cost.\hfill$\square$
\end{rem}

\subsection{Communication Efficiency}\label{sec::com_eff}

{\color{blue}
Let $C_{\mathrm{CG}}(T)$ and $C_{\mathrm{ATCG}}(T)$ denote the
cumulative number of feature embeddings uploaded to the server
through step $T$ under CG and \textit{ATCG}, respectively.
In \textit{ATCG}, a feature embedding is transmitted only when
its element first enters an active set, so communication is
governed by the growth of $\{\mathcal{A}_i\}_{i=1}^N$.
Potentially, standard \textit{CG} can select a new element
per partition at every iteration as $\mathbf{x}$ evolves, so
$C_{\mathrm{CG}}(T)\to|\mathcal{P}|$ as $T\to\infty$;
\textit{ATCG} prevents this through its per-partition threshold
mechanism: the expansion step in Algorithm~\ref{alg:atcg}
fires only when $\eta_i(t)<\tau$, directly gating which
embeddings are ever transmitted.

\begin{lem}[Communication Dominance]\label{lem:comm_dom}
Let $j_i^{\mathrm{CG}}(t)\in\arg\max_{j\in\mathcal{P}_i}
[\nabla F(\mathbf{x}(t))]_j$ denote the CG oracle selection
in partition~$i$ at iteration~$t$ along the \textit{ATCG}
trajectory, so that
$C_{\mathrm{CG}}(T) = \sum_{i=1}^N
\bigl|\bigcup_{t=0}^{T-1}\{j_i^{\mathrm{CG}}(t)\}\bigr|$.
Then $C_{\mathrm{ATCG}}(T)\le C_{\mathrm{CG}}(T)$
for all $T\ge 1$.
\end{lem}

\begin{proof}
Fix partition~$i$. Whenever \textit{ATCG} expands
$\mathcal{A}_i$ at iteration~$t$, $\eta_i(t)<\tau\le 1$,
so $\max_{j\in\mathcal{A}_i}[\nabla F]_j <
\max_{j\in\mathcal{P}_i}[\nabla F]_j$; hence
$j_i^{\mathrm{CG}}(t)\notin\mathcal{A}_i(t)$ and
\textit{ATCG} selects
\[
\arg\max_{j\in\mathcal{P}_i\setminus\mathcal{A}_i(t)}
[\nabla F(\mathbf{x}(t))]_j
= j_i^{\mathrm{CG}}(t),
\]
up to consistent tie-breaking.
Therefore
$\mathcal{A}_i(T)\subseteq
\bigcup_{t=0}^{T-1}\{j_i^{\mathrm{CG}}(t)\}$,
and summing over all partitions gives
$C_{\mathrm{ATCG}}(T)\le C_{\mathrm{CG}}(T)$.\boxend
\end{proof}

Since $\eta_i(t)\in[0,1]$ is computed from $K$ Monte Carlo
gradient estimates via~\eqref{eq::grad}, it fluctuates around
a nominal value $\bar{\eta}_i(t)$ whose variability decreases
as $K$ grows. To quantify the role of $\tau$ explicitly, we
adopt the following one-sided bound as a modeling assumption:
\begin{equation}\label{eq::threshold_prob}
\mathbb{P}\!\left(\eta_i(t)<\tau\right)
\;\le\;
\Phi\!\left(
\frac{\tau-\bar{\eta}_i(t)}{\sigma_i}
\right),
\quad \forall\,i,t,\tau,
\end{equation}
where $\Phi$ is the standard Gaussian CDF and $\sigma_i>0$
captures the variability of $\eta_i(t)$. This is a
conservative tail bound on the activation probability, not
a claim that $\eta_i(t)$ is Gaussian: when
$\tau\ll\bar{\eta}_i(t)$ violations are rare, and when $\tau$
increases the bound grows monotonically, reflecting the
stricter coverage~requirement. %Next, we quantify how the probability of threshold violations governs the expected communication cost of \textit{ATCG}.

\begin{lem}[Expected Communication]\label{lem:exp_comm}
Under the threshold-violation model~\eqref{eq::threshold_prob}, let
\(T>1\). Then, 
{\small \[
\mathbb{E}\!\left[C_{\mathrm{ATCG}}(T)\right]
\le
\min\!\left\{
\mathbb{E}\!\left[C_{\mathrm{CG}}(T)\right],
N
\!+\!\sum_{t=1}^{T-1}\sum_{i=1}^N
\Phi\!\left(
\frac{\tau-\bar{\eta}_i(t)}{\sigma_i}
\right)\!
\right\}.
\]}
\end{lem}

\begin{proof}
Define $Z_{i,t}=\mathbf{1}\{\eta_i(t)<\tau,\,
\mathcal{A}_i(t)\ne\mathcal{P}_i\}$.
Since \(\mathcal{A}_i(0)=\emptyset\), \textit{ATCG} activates
one largest-marginal element from each partition at the first iteration,
which accounts for \(N\) initial transmitted feature embeddings. Hence, for \(T>1\)
$C_{\mathrm{ATCG}}(T)=N+\sum_{t=1}^{T-1}\sum_{i=1}^N Z_{i,t}$.
Taking expectations and applying
\(
\mathbb{P}\!\left(\eta_i(t)<\tau,\;
\mathcal{A}_i(t)\ne\mathcal{P}_i\right)
\;\le\;
\mathbb{P}\!\left(\eta_i(t)<\tau\right)
\;\le\;
\Phi\!\left(\frac{\tau-\bar{\eta}_i(t)}{\sigma_i}\right)
\)
yields the second bound.
Taking expectations in Lemma~\ref{lem:comm_dom}
gives the first.
Combining both bounds via the minimum completes the proof.\boxend
\end{proof}
This bound highlights that communication is driven not by the full gradient dynamics, but by rare excursions where the active set fails to capture sufficient marginal gain, so when $\bar{\eta}_i(t)$ remains above $\tau$ most of the time, the communication cost stays close to its minimum.

Next, we characterize the minimum
achievable communication savings. For this, we define the \textit{partition curvature}
\begin{equation*}
    c_i = 1 - \min_{\mathcal{S}\subset\mathcal{P},\;
    p\in\mathcal{P}_i\setminus\mathcal{S}}
    \frac{f(\mathcal{S}\cup\{p\})-f(\mathcal{S})}{f(\{p\})}
\end{equation*}
which measures marginal-gain deterioration for elements of
partition~$i$; under low curvature, a highly informative element
in $\mathcal{A}_i$ remains competitive as $\mathbf{x}$ evolves,
as formalized below.


\begin{lem}[Communication Complexity]\label{lem:comm}
Let $C_{\mathrm{ATCG}}(T)=\sum_{i=1}^{N}|\mathcal{A}_i(T)|$.
For any $i\in[N]$, if $\tau\le 1-c_i$, then
$\eta_i(t)\ge\tau$ for all $t\ge 1$,
so $|\mathcal{A}_i(T)|=1$ for all $T\ge 1$.
Moreover, if $\tau\le 1-\max_{i\in[N]}\{c_i\}$, then
$C_{\mathrm{ATCG}}(T)=N$ for all $T\ge 1$,
attaining the minimum possible communication of one
embedding per~partition.
\end{lem}

\begin{proof}
At $t=0$, $\mathcal{A}_i=\emptyset$ so $\eta_i=0<\tau$,
and \textit{ATCG} activates
$j_i^\circ=\arg\max_{j\in\mathcal{P}_i}f(\{j\})$
in each partition.
We show $\eta_i(t)\ge 1-c_i\ge\tau$ for all $t\ge 1$,
so the expansion condition is never triggered again. Since $j_i^\circ\in\mathcal{A}_i(t)$ for all $t\ge 1$
by monotonicity of the active sets,
\begin{equation*}
    \max_{j\in\mathcal{A}_i(t)}[\nabla F(\mathbf{x}(t))]_j
    \;\ge\; [\nabla F(\mathbf{x}(t))]_{j_i^\circ}
    \;\ge\; (1-c_i)\,f(\{j_i^\circ\}),
\end{equation*}
where the second inequality uses the partition curvature
lower bound $[\nabla F(\mathbf{x})]_j\ge(1-c_i)f(\{j\})$
for $j\in\mathcal{P}_i$, obtained by taking expectations
in $f(\mathcal{S}\cup\{j\})-f(\mathcal{S})\ge(1-c_i)f(\{j\})$
over $\mathcal{S}=\mathcal{R}(\mathbf{x})$~\eqref{eq::grad}.
Submodularity (set $\mathcal{S}=\emptyset$) and expectations
via~\eqref{eq::grad} give
$[\nabla F(\mathbf{x}(t))]_j\le f(\{j\})\le f(\{j_i^\circ\})$
for all $j\in\mathcal{P}_i$:
\begin{equation*}
  \frac{\max_{j\in\mathcal{A}_i(t)}
           [\nabla F(\mathbf{x}(t))]_j}
          {\max_{j\in\mathcal{P}_i}
           [\nabla F(\mathbf{x}(t))]_j}
    \;\ge\;
    \frac{(1-c_i)\,f(\{j_i^\circ\})}{f(\{j_i^\circ\})}
    = 1-c_i.
\end{equation*}
Therefore,   $\eta_i(t)\geq 1-c_i\;\ge\;\tau.$
The expansion condition is never triggered after $t=0$,
so $|\mathcal{A}_i(T)|=1$ for all $T\ge 1$.
Applying this to every $i\in[N]$ under
$\tau\le 1-\max_i c_i$ gives $C_{\mathrm{ATCG}}(T)=N$.\boxend
\end{proof}

Combined with Theorem~\ref{thm:atcg_curvature},
Lemma~\ref{lem:comm} completes the Pareto picture
established in Remark~\ref{rem:pareto}:
since $c_i\le c$ for all $i$, the per-partition bound
gives $1-\max_i c_i\ge 1-c$, strictly widening the
safe regime relative to the global curvature bound,
and as $\max_i c_i\to 0$ this expands to $\tau\in(0,1]$,
permitting $C_{\mathrm{ATCG}}(T)=N$ and near-optimal
$(1-1/e)$ performance~simultaneously.
}


==> Algorithm_design_v3.tex <==
\section{Problem Definition}\label{sec::problem}

Consider optimization problem~\eqref{eq::canonical_prob} where the 
ground set $\mathcal{P} = \bigcup_{i=1}^{N}\mathcal{P}_i$ is a finite 
set partitioned into $N$ disjoint subsets, where $\mathcal{P}_i$ 
represents the candidate elements associated with agent $i$. The utility 
function $f:2^{\mathcal{P}}\to\mathbb{R}_{+}$ is \emph{submodular}, 
i.e., it satisfies the diminishing-returns property:
\begin{equation}
f(\mathcal{A}\cup\{e\})-f(\mathcal{A})\geq 
f(\mathcal{B}\cup\{e\})-f(\mathcal{B}),
\quad \forall\,\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{P},
\; e\notin\mathcal{B},
\end{equation}
and \emph{monotone}, i.e., $f(\mathcal{A})\leq f(\mathcal{B})$ 
whenever $\mathcal{A}\subseteq\mathcal{B}$. The matroid constraint is 
a \emph{partition matroid}~\footnote{In 
Fig.~\ref{fig:forward_gradient}, the matroid constraint is a partition 
matroid with non-overlapping local ground sets defined for each agent 
$i\in\{1,\cdots,N\}$ as $\mathcal{P}_i = \{(i,b)\mid b\in\mathcal{B}_i\}$, 
where $\mathcal{B}_i$ is the set of deployment choices of agent $i$.} 
that enforces at most one element per partition, defining the family 
of feasible sets:
\begin{equation}\label{eq::partition_matroid}
\mathcal{I}=\big\{\mathcal{S}\subseteq\mathcal{P}\;\big|\;
|\mathcal{S}\cap\mathcal{P}_i|\leq 1,\;\forall\,i\in[N]\big\}.
\end{equation}

Following~\cite{calinescu2011maximizing}, to 
solve~\eqref{eq::canonical_prob} tractably, we optimize the 
multilinear extension $F(\mathbf{x})$ defined 
in~\eqref{eq::multi_linear} over the \emph{matroid polytope}
\begin{equation}\label{eq::polytope}
\mathcal{M}=\Big\{\mathbf{x}\in[0,1]^{n}\;\Big|\;
\textstyle\sum_{j\in\mathcal{P}_i}[\mathbf{x}]_j
\leq 1,\;\forall\,i\in[N]\Big\},
\end{equation}
the convex hull of the feasible indicator vectors, yielding the 
relaxed problem
\begin{equation}\label{eq::cont}
\max_{\mathbf{x}\in\mathcal{M}}\;F(\mathbf{x}).
\end{equation}
The CG algorithm~\cite{calinescu2011maximizing} 
solves~\eqref{eq::cont} by initializing $\mathbf{x}(0)=\mathbf{0}$ 
and iterating
\begin{equation}\label{eq::CG_update}
\mathbf{v}(t)=\operatorname*{arg\,max}_{\mathbf{v}\in\mathcal{M}}\;
\mathbf{v}^{\!\top}\nabla F(\mathbf{x}(t)),
\qquad
\mathbf{x}\!\left(t+\tfrac{1}{T}\right)=
\mathbf{x}(t)+\tfrac{1}{T}\,\mathbf{v}(t),
\end{equation}
for $T$ steps, where the gradient of $F$ admits the stochastic 
representation
\begin{equation}\label{eq::grad}
[\nabla F(\mathbf{x})]_j = 
\mathbb{E}\big[f(\mathcal{R}(\mathbf{x})\cup\{j\})
-f(\mathcal{R}(\mathbf{x})\setminus\{j\})\big],
\end{equation}
estimated in practice via Monte Carlo sampling. A lossless rounding 
step then recovers a feasible $\mathcal{S}\in\mathcal{I}$, achieving 
the $(1-1/e)$-approximation 
guarantee~\cite{calinescu2011maximizing}.

Without loss of generality, we identify $\mathcal{P}=\{1,\ldots,n\}$ 
with $n\triangleq|\mathcal{P}|$, where the elements of each block 
$\mathcal{P}_i$ occupy a contiguous range of indices. Under this 
labeling, the $j$-th component of the decision vector and its 
corresponding gradient entry are written as $[\mathbf{x}]_j$ and 
$[\nabla F(\mathbf{x})]_j$ for $j\in\mathcal{P}_i$, with the owning 
block $i$ implicitly determined by the index $j$.

The non-negativity of the multilinear gradient for monotone 
submodular functions, combined with the blockwise structure of the 
matroid polytope~\eqref{eq::polytope}, ensures that the linear oracle 
in~\eqref{eq::CG_update} decomposes blockwise. Specifically, for 
each block $i$, the element of $\mathcal{P}_i$ with the largest 
gradient value is
\begin{equation}\label{eq::oracle_decomp}
j_i^\star(t) \in \operatorname*{arg\,max}_{j\in\mathcal{P}_i}
[\nabla F(\mathbf{x}(t))]_j,
\end{equation}
and one realization of the optimal ascent direction is
\begin{equation}\label{eq::ascent_decomp}
\mathbf{v}^\star(t) = \sum_{i=1}^{N}\,\mathbf{e}_{j_i^\star(t)}
\;\in\mathcal{M},
\end{equation}
where $\mathbf{e}_j\in\mathbb{R}^n$ denotes the $j$-th standard 
basis vector, so that $[\mathbf{v}^\star(t)]_{j_i^\star}=1$ for each 
$i\in[N]$ and zero otherwise. At each step, exactly one entry of 
$\mathbf{x}$ per block is incremented by $\tfrac{1}{T}$. This 
blockwise separability makes CG naturally amenable to a 
server-assisted distributed realization.

\subsection{Server-Assisted Distributed Realization}

We consider a server-assisted architecture\footnote{The 
server-assisted architecture bears structural resemblance to 
federated learning: agents retain local data ownership, communicate 
only task-relevant updates, and coordinate through a central 
aggregator. However, unlike FedAvg---where the server passively 
averages local model updates---the server here actively performs 
gradient estimation by sampling from $\mathcal{R}(\mathbf{x})$ over 
all currently active elements, making it the primary computational 
node rather than a lightweight coordinator.} in which $N$ agents, 
each owning block $\mathcal{P}_i$, collaborate through a central 
server to execute CG in parallel. Each agent $i$ initializes and 
maintains its own local sub-vector $\mathbf{x}_i(0)=\mathbf{0}$ of 
the global decision vector 
$\mathbf{x}=[\mathbf{x}_1^\top,\ldots,\mathbf{x}_N^\top]^\top$, 
and evolves it independently using only the block gradient 
$\{[\nabla F(\mathbf{x}(t))]_j\}_{j\in\mathcal{P}_i}$ received 
from the server. One iteration of the distributed CG proceeds as 
follows:
\begin{enumerate}
    \item \textit{Local oracle}: Since the partition-matroid polytope 
    decouples across blocks~\eqref{eq::ascent_decomp}, each agent $i$ 
    computes its local ascent direction independently. Given the block 
    gradient 
    $\{[\nabla F(\mathbf{x}(t))]_j\}_{j\in\mathcal{P}_i}$ 
    received from the server, agent $i$ identifies $j_i^\star$ 
    via~\eqref{eq::oracle_decomp}, sets 
    $[\mathbf{v}_i]_{j_i^\star}=1$ and zero otherwise, and updates 
    its sub-vector:
    \begin{equation*}
    [\mathbf{x}_i]_{j_i^\star} \leftarrow 
    [\mathbf{x}_i]_{j_i^\star} + \tfrac{1}{T}.
    \end{equation*}
    \item \textit{Upload}: Agent $i$ transmits its updated 
    $\mathbf{x}_i(t+\tfrac{1}{T})$ to the server. If $j_i^\star$ 
    transitions from inactive to active (i.e., 
    $[\mathbf{x}_i]_{j_i^\star}$ becomes non-zero for the first 
    time), agent $i$ also transmits the feature embedding of element 
    $j_i^\star$ to the server. At most one new feature embedding is 
    uploaded per block per iteration.
    \item \textit{Server gradient estimation}: The server assembles 
    the global state $\mathbf{x}(t+\tfrac{1}{T})$ from all agents' 
    sub-vectors, draws $K$ Monte Carlo samples of 
    $\mathcal{R}(\mathbf{x})$ using the feature embeddings of all 
    currently active elements, and empirically estimates 
    $[\nabla F(\mathbf{x})]_j$ for all $j\in\mathcal{P}_i$ 
    via~\eqref{eq::grad}.
    \item \textit{Gradient download}: The server returns 
    $\{[\nabla F(\mathbf{x}(t+\tfrac{1}{T}))]_j\}_{j\in\mathcal{P}_i}$ 
    to each agent $i$ for use in the next iteration.
\end{enumerate}
This architecture realizes the centralized CG algorithm through 
parallel local computation and server-mediated gradient aggregation. 
The communication overhead is governed by the number of elements that 
ever become active: each time $[\mathbf{x}_i]_j$ transitions from 
zero to non-zero, the feature embedding of element $j$ must be 
transmitted to and held by the server for gradient sampling. Since 
the gradient estimate in Step~3 requires evaluating 
$f(\mathcal{R}(\mathbf{x})\cup\{j\})$ over all active elements in 
$\mathcal{R}(\mathbf{x})$, every activated element contributes to 
the server's sampling cost. As CG progresses and $\mathbf{x}$ becomes 
dense, this forces the transmission of feature data for nearly every 
element of $\mathcal{P}$, resulting in communication overhead that 
scales with $|\mathcal{P}|$ rather than the size of any local final 
selection. Controlling which elements ever become active---and 
therefore which feature embeddings are ever uploaded---is therefore 
the central motivation for \textit{ATCG}.

==> Objective_statement_v1.tex <==
\section{Problem Definition}\label{sec::problem}

Consider optimization problem~\eqref{eq::canonical_prob} where the 
ground set $\mathcal{P} = \bigcup_{i=1}^{N}\mathcal{P}_i$ is a finite 
set, consisted of partitioned  $N$ disjoint subsets, where partition $\mathcal{P}_i$ 
represents the candidate elements associated with agent $i$. The utility 
function $f:2^{\mathcal{P}}\to\mathbb{R}_{+}$ is \emph{submodular}, 
i.e., it satisfies the diminishing-returns property:
\begin{equation}
f(\mathcal{A}\cup\{e\})-f(\mathcal{A})\geq 
f(\mathcal{B}\cup\{e\})-f(\mathcal{B}),
~~ \forall\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{P},
\; e\notin\mathcal{B},
\end{equation}
and \emph{monotone}, i.e., $f(\mathcal{A})\leq f(\mathcal{B})$ 
whenever $\mathcal{A}\subseteq\mathcal{B}$. The matroid constraint is 
a \emph{partition matroid}~\footnote{In Fig.~\ref{fig:forward_gradiant}, the matroid constraint is a partition matroid, with non-overlapping local ground sets defined for each agent $i\in[N]=\{1,\cdots,N\}$ as $\mathcal{P}_i = \{(i, b) \, | \, b \in \mathcal{B}_i\}$, where $\mathcal{B}_i$ is the deployment choices of agent $i$} 
that enforces at most $\kappa_i$ elements 
may be selected from each partition, defining the family of feasible sets:
\begin{equation}\label{eq::partion_matroid}
\mathcal{I}=\big\{\mathcal{S}\subseteq\mathcal{P}\;\big|\;
|\mathcal{S}\cap\mathcal{P}_i|\leq1,\;\forall\,i\in[N]\big\}.
\end{equation}

Following~\cite{calinescu2011maximizing}, to solve~\eqref{eq::canonical_prob} 
tractably, we optimize the multilinear extension $F(\mathbf{x})$ 
defined in~\eqref{eq::multi_linear} over the \emph{matroid polytope}
\begin{equation}\label{eq::polytope}
\mathcal{M}=\Big\{\mathbf{x}\in[0,1]^{|\mathcal{P}|}\;\Big|\;
\textstyle\sum_{j\in\mathcal{P}_i}[\mathbf{x}]_j
\leq 1,\;\forall\,i\in[N]\Big\},
\end{equation}
the convex hull of the feasible indicator vectors, yielding the 
relaxed problem
\begin{equation}\label{eq::cont}
\max_{\mathbf{x}\in\mathcal{M}}\;F(\mathbf{x}).
\end{equation}
The CG algorithm~\cite{calinescu2011maximizing} solves~\eqref{eq::cont} 
by initializing $\mathbf{x}(0)=\mathbf{0}$ and following the 
continuous-time ascent flow for $t\in[0,1]$
\begin{equation}\label{eq::CG_update}
\mathbf{v}(t)=\operatorname*{arg\,max}_{\mathbf{v}\in\mathcal{M}}\;
\mathbf{v}^{\!\top}\nabla F(\mathbf{x}(t)),
\qquad
\frac{\mathrm{d}}{\mathrm{d}t}\mathbf{x}(t)=\mathbf{v}(t),
\end{equation}
where the gradient of $F$ admits the stochastic representation
\begin{equation}\label{eq::grad}
[\nabla F(\mathbf{x})]_j = 
\mathbb{E}\big[f(\mathcal{R}(\mathbf{x})\cup\{j\})
-f(\mathcal{R}(\mathbf{x})\setminus\{j\})\big].
\end{equation}
A lossless rounding step using $\vect{x}(1)$ then recovers a feasible 
$\mathcal{S}\in\mathcal{I}$, achieving the 
$(1-1/e)$-approximation guarantee~\cite{calinescu2011maximizing}. 
In practice, the continuous flow~\eqref{eq::CG_update} is 
discretized into $T$ steps
\begin{equation}\label{eq::CG_disc}
\mathbf{x}\!\left(t+\tfrac{1}{T}\right)=
\mathbf{x}(t)+\tfrac{1}{T}\,\mathbf{v}(t),
\end{equation}
with the gradient estimated via Monte Carlo 
sampling~\cite{calinescu2011maximizing}.

Without loss of generality, we let $\mathcal{P}=\{1,\ldots,n\}$ 
with $n\triangleq|\mathcal{P}|$, where the elements of each partition 
$\mathcal{P}_i$ occupy a contiguous range of indices. Under this 
labeling, the $j$-th component of the probability membership  vector and its 
corresponding gradient entry are written as $[\mathbf{x}]_j$ and 
$[\nabla F(\mathbf{x})]_j$ for $j\in\mathcal{P}_i$, with the owning 
partition $i$ implicitly determined by the index $j$.


The non-negativity of the multilinear gradient for monotone
submodular functions, combined with the partition-wise structure
of the matroid polytope~\eqref{eq::polytope}, ensures that
the linear oracle in~\eqref{eq::CG_update} decomposes
partition-wise. The oracle to choose $\vect{v}(t)$, reduces
to identifying, within each partition $i$, the single element
with the largest gradient value:
\begin{equation}\label{eq::oracle_decomp}
    j_i^\star = \operatorname*{arg\,max}_{j \in \mathcal{P}_i}
    [\nabla F(\mathbf{x}(t))]_j,
\end{equation}
and the optimal ascent direction $\mathbf{v}^\star(t) \in \mathcal{M}$ is
defined componentwise as
\begin{equation}\label{eq::ascent_decomp}
    [\mathbf{v}^\star(t)]_j =
    \begin{cases}
        1 & \text{if } j = j_i^\star \text{ for some } i \in [N], \\
        0 & \text{otherwise,}
    \end{cases}
\end{equation}
so that exactly one entry of $\mathbf{x}$ per partition is
incremented by $\tfrac{1}{T}$ at each step, with the
updated entry identified by the global index $j_i^\star \in
\mathcal{P}_i$. This partitionwise separability makes CG
naturally amenable to a server-assisted distributed
realization.

\subsection{Server-Assisted Distributed Realization}

We consider a server-assisted architecture\footnote{The
server-assisted architecture bears structural resemblance to
federated learning: agents retain local data ownership, communicate
only task-relevant updates, and coordinate through a central
aggregator. However, unlike FedAvg \cite{mcmahan2017communication}---where the server passively
averages local model updates---the server here actively performs
gradient estimation by sampling from $\mathcal{R}(\mathbf{x})$ over
all currently active elements, making it the primary computational
node rather than a lightweight coordinator.} in which $N$ agents,
each owning partition $\mathcal{P}_i$, collaborate through a central
server to execute CG in parallel. Each agent $i$ initializes and
maintains its own local sub-vector $\mathbf{x}_i(0)=\mathbf{0}$ of
the global decision vector
$\mathbf{x}=[\mathbf{x}_1^\top,\ldots,\mathbf{x}_N^\top]^\top$,
and evolves it independently using only the block gradient
$\{[\nabla F(\mathbf{x}(t))]_j\}_{j\in\mathcal{P}_i}$ received
from the server. Each iteration of the distributed CG is formalized
in Algorithm~\ref{alg:cg}: the server estimates the gradient over
all currently active elements and broadcasts the relevant block
gradients to each agent; each agent independently solves its local
oracle~\eqref{eq::oracle_decomp} and updates its sub-vector; agents
upload their updated sub-vectors together with the feature embedding
of any newly activated element; and the server reassembles the
global state for the next iteration.

This architecture realizes the centralized CG algorithm through
parallel local computation and server-mediated gradient aggregation.
The communication overhead is governed by the number of elements
that ever become active: each time $[\mathbf{x}_i]_{j}$ transitions
from zero to non-zero, the feature embedding of element $j$ must be
transmitted to and held by the server for gradient sampling. Since
gradient estimation requires evaluating
$f(\mathcal{R}(\mathbf{x})\cup\{j\})$ over all active elements
in $\mathcal{R}(\mathbf{x})$, every activated element contributes
to the server's sampling cost. As CG progresses and $\mathbf{x}$
becomes dense, this forces the transmission of feature data for
nearly every element of $\mathcal{P}$, resulting in communication
overhead that scales with $|\mathcal{P}|$ rather than the $N$
locally selected elements. Controlling which elements ever become
active---and therefore which feature embeddings are ever
uploaded---is therefore the central motivation for \textit{ATCG}.


%--- SERVER-ASSISTED CG BASELINE ALGORITHM ---%
\begin{algorithm}[t]\footnotesize
\caption{\textbf{CG} in Server-Assisted
Realization}}
\label{alg:cg}
\begin{algorithmic}[1]\footnotesize
\Require Ground set
$\mathcal{P}=\bigcup_{i=1}^N\mathcal{P}_i$ with
disjoint partitions $\mathcal{P}_i$; horizon $T$;
number of samples $K$
\State \textbf{[Server]}\; $\mathbf{x}\leftarrow\mathbf{0}$;\;
active embedding set $\mathcal{E}\leftarrow\emptyset$
\State \textbf{[Agent $i$, $\forall i$]}\;
$\mathbf{x}_i\leftarrow\mathbf{0}$
\For{$t=0,1,\ldots,T-1$}
    \State \textbf{[Server]}\; Estimate
    $\mathbf{g}\approx\nabla F(\mathbf{x})$ using $K$ MC
    samples via~\eqref{eq::grad} over $\mathcal{E}$
    \hfill$\triangleright$ \textit{Gradient estimation}
    \State \textbf{[Server$\,\to\,$Agent $i$]}\; Send
    $\{[\mathbf{g}]_j\}_{j\in\mathcal{P}_i}$ to each agent $i$
    \hfill$\triangleright$ \textit{Gradient download}
    \For{$i=1,\ldots,N$}
    \hfill$\triangleright$ \textit{Local oracle (parallel)}
        \State \textbf{[Agent $i$]}\;
        $j_i^\star\in\operatorname*{arg\,max}_{j\in\mathcal{P}_i}
        [\mathbf{g}]_j$
        \hfill via~\eqref{eq::oracle_decomp}
        \State \textbf{[Agent $i$]}\;
        $[\mathbf{x}_i]_{j_i^\star}\leftarrow
        [\mathbf{x}_i]_{j_i^\star}+\tfrac{1}{T}$
    \EndFor
    \For{$i=1,\ldots,N$}
    \hfill$\triangleright$ \textit{Upload (parallel)}
        \State \textbf{[Agent $i\,\to\,$Server]}\; Transmit
        $\mathbf{x}_i(t+\tfrac{1}{T})$
        \If{$[\mathbf{x}_i]_{j_i^\star}$ becomes non-zero
        for the first time}
            \State \textbf{[Agent $i\,\to\,$Server]}\; Transmit
            embedding of $j_i^\star$;\;
            $\mathcal{E}\leftarrow\mathcal{E}\cup\{j_i^\star\}$
        \EndIf
    \EndFor
    \State \textbf{[Server]}\; Assemble
    $\mathbf{x}(t+\tfrac{1}{T})=
    [\mathbf{x}_1^\top,\ldots,\mathbf{x}_N^\top]^\top$
\EndFor
\State \textbf{[Server]}\; \textbf{Rounding:} Round $\mathbf{x}$
to feasible $\mathcal{S}\in\mathcal{I}$
\State \Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

% \footnotetext{The theoretical analysis is stated in
% terms of the exact gradient of the multilinear
% extension. In the practical implementation and
% numerical experiments, this gradient is approximated
% via Monte Carlo sampling as in~\eqref{eq::grad}.
% The algorithms above should therefore be interpreted
% as sampled implementations of CG and \textit{ATCG},
% whereas the theoretical guarantees are derived for
% their exact-gradient counterparts.}

==> intro_1.tex <==
\section{Introduction}

Submodular maximization has emerged as a cornerstone of modern discrete 
and combinatorial optimization, underpinning a wide range of applications 
in machine learning, control, and networked decision-making~\cite{krause2014submodular, 
nemhauser1978analysis, calinescu2011maximizing, bach2013learning}. 
Submodular functions naturally model notions of diversity, 
representativeness, and information coverage, and thus appear in problems 
such as sensor placement~\cite{krause2008near}, data 
summarization~\cite{lin2011class}, influence maximization~\cite{kempe2003maximizing}, 
and active learning~\cite{golovin2011adaptive}.

\begin{figure}[t]
\centering
    \includegraphics[scale=0.23]{Fig/schem.png}
\caption{{\small Spatial comparison of the early-commitment effect in a 
2D sensor placement task. The objective is to select deployment points 
(solid circles) from candidates (red $\times$) to cover a clustered data 
distribution (blue dots) under partition-matroid constraints (colored 
ellipses). (i)~Sequential Greedy: myopic selection leads the first agent 
to a central median point, producing a locally optimal but globally 
suboptimal arrangement that fails to capture the four distinct clusters. 
(ii)~Continuous Greedy: fractional allocations evolve along a continuous 
ascent trajectory, allowing agents to avoid premature commitment and 
settle on a superior arrangement that accurately partitions and covers 
the data distribution.}}
    \label{fig:forward_gradiant}
\end{figure}

A central problem in this area is constrained submodular maximization 
under a \emph{matroid constraint}, which generalizes independence 
structures such as cardinality, partition, or budget 
limits~\cite{calinescu2011maximizing}. The canonical formulation with 
utility function $f:2^\mathcal{P}\to\mathbb{R}_{+}$ is
\begin{equation}\label{eq::canonical_prob}
\max_{\mathcal{S} \in \mathcal{I}} f(\mathcal{S}),
\end{equation}
where $\mathcal{I}$ denotes the independent sets of a matroid on ground 
set $\mathcal{P}$. This problem is NP-hard.

The \emph{Sequential Greedy (SG)} algorithm~\cite{nemhauser1978analysis, 
fisher2009analysis} offers a classical polynomial-time solution by 
iteratively selecting the element with the largest marginal gain in 
$f(\mathcal{S})$, starting from the empty set. Despite its simplicity 
and scalability, SG achieves only a $(1/2)$-approximation for monotone 
submodular functions under general matroid constraints, as its discrete, 
myopic selections can lead to locally optimal but globally suboptimal 
solutions. The \emph{Continuous Greedy (CG)} algorithm~\cite{calinescu2011maximizing} 
closes this gap by optimizing over the \emph{multilinear extension} of $f$,
$$
F(x) = \mathbb{E}[f(\mathcal{R}(x))],
$$
where $x\in[0,1]^{|\mathcal{P}|}$ and $\mathcal{R}(x)$ includes each 
element $i$ independently with probability $x_i$. By following a 
continuous ascent trajectory within the matroid polytope, CG achieves 
the optimal $(1-1/e)$ approximation, with the final solution recovered 
via a lossless rounding step. Intuitively, rather than making 
irrevocable discrete commitments, CG maintains a fractional 
representation that gradually evolves toward a balanced allocation of 
probabilities across competing elements, thereby mitigating the 
early-commitment effect inherent to SG. This qualitative difference is 
illustrated in Fig.~\ref{fig:forward_gradiant}.

Despite its theoretical elegance and improved approximation guarantee, 
deploying CG in distributed or networked systems introduces significant 
computational and communication challenges. Each iteration requires 
evaluating or estimating the gradient $\nabla F(x)$, which depends on 
the contribution of all elements of the ground set $\mathcal{P}$---which 
may be distributed among agents across the network, as in the partition 
matroid case. Consequently, the distributed realization of CG 
(e.g.,~\cite{AM-HH-AK:18, rezazadeh2023distributed}) involves not only 
consensus on the decision vector $x$ among neighboring agents, but also 
the exchange of gradient-related statistics and local ground set 
embeddings across the network---leading to substantial communication 
overhead, latency, and exposure of local data across agents. These costs 
stand in contrast to SG, which requires no such data exchange, albeit at 
the price of a suboptimal $(1/2)$-approximation guarantee.

This work proposes a methodology to reduce the communication overhead 
of CG in distributed settings, demonstrated over a server-assisted 
implementation of the continuous greedy algorithm under a 
partition-matroid structure. Each agent maintains and updates a local 
block of the decision vector $x$, while a central server aggregates 
and broadcasts information for global gradient estimation. 
Communication overhead arises from two coupled sources: 
(\textit{i})~each agent must share its local block $\mathbf{x}_i$ to 
maintain a consistent global state for estimating $\nabla F(x)$, and 
(\textit{ii})~whenever a component of $x_i$ becomes non-zero---indicating 
element activation---the agent must also transmit the associated data 
point to the server for redistribution. Both transmissions are necessary 
for accurate gradient computation, and their combined frequency directly 
governs the system's communication load. While the proposed thresholding 
framework naturally extends to other distributed 
topologies~\cite{AM-HH-AK:18, rezazadeh2023distributed}, we limit the 
scope of this work to the server-assisted setting as a principled first 
step toward communication-efficient distributed submodular optimization.

To address this overhead, we propose \texttt{CG-$\eta$-Online}, a 
threshold-based variant of CG that reduces both computational and 
communication costs in the server-assisted distributed setting. The 
core idea is to allow each agent to selectively restrict its gradient 
evaluations to a small, dynamically expanding active subset, avoiding 
unnecessary transmissions when the current subset already provides 
sufficient optimization progress. This selective activation preserves 
the near-optimality of continuous greedy while substantially reducing 
both gradient evaluations and inter-agent information exchange.

\emph{Related work}: Thresholding and hard-threshold operators have a 
rich history in optimization and signal processing. The compressed 
sensing literature has developed \emph{iterative hard thresholding} 
(IHT) and its variants to enforce sparsity constraints~\cite{pan2017convergent, 
yuan2014gradient, foucart2011hard}, and related works apply constrained 
thresholded updates in nonconvex optimization~\cite{liu2020between}. 
While superficially similar in name, our mechanism differs fundamentally 
in both goal and operation: \cite{pan2017convergent} targets 
sparsity-constrained minimization via Armijo-type step sizes; 
\cite{yuan2014gradient} enforces sparsity per iteration via thresholded 
projection onto candidate support sets; \cite{foucart2011hard} selects 
signal support under linear measurement models; and \cite{liu2020between} 
alternates thresholding with gradient descent to balance convergence 
stability and sparsity. In contrast, \texttt{CG-$\eta$-Online} uses 
thresholding not to enforce sparsity, but to \emph{adaptively decide 
when to expand} the active set for gradient evaluation---guided by a 
ratio of marginal gains, operating blockwise under a partition matroid, 
and motivated by communication efficiency rather than continuous 
sparse minimization.

Scalability in submodular optimization has also been pursued through 
two complementary directions. \emph{Lazy greedy}~\cite{minoux1978accelerated, 
leskovec2007cost} accelerates SG by caching marginal gain upper bounds 
to skip redundant evaluations, but inherits the $(1/2)$-approximation 
ceiling of SG and does not extend to the continuous domain. 
MapReduce-based approaches~\cite{mirzasoleiman2013distributed, 
kumar2015fast} achieve one-round communication efficiency through a 
partition-and-merge paradigm, but incur approximation loss---typically 
$(1/4)$ or worse---due to the absence of global coordination during 
local selection. \texttt{CG-$\eta$-Online} operates entirely within the 
CG framework, preserving the $(1-1/e)$ guarantee while achieving 
communication efficiency through the adaptive $\eta$-threshold rule, 
without partitioning computation or sacrificing near-optimality.

\emph{Statement of contributions}: This paper introduces a 
threshold-driven mechanism for submodular maximization under 
partition-matroid constraints that bridges the gap between theoretical 
optimality and communication efficiency. Unlike static or pre-defined 
truncation schemes, \texttt{CG-$\eta$-Online} dynamically expands 
active sets based on local progress indicators, directing gradient and 
communication effort toward the most informative elements while 
retaining the monotone ascent property of continuous greedy dynamics. 
The main contributions are:
\begin{itemize}
    \item A novel threshold-based continuous greedy algorithm that 
    adaptively expands active sets based on per-agent progress indicators;
    \item Theoretical analysis establishing approximation guarantees 
    that incorporate both threshold parameters and function curvature;
    \item Empirical validation demonstrating favorable trade-offs 
    between solution quality and computational efficiency.
\end{itemize}

==> intro_old.tex <==
\section{Introduction}
Submodular maximization has emerged as a cornerstone of modern discrete and combinatorial optimization, underpinning a wide range of applications in machine learning, control, and networked decision-making~\cite{krause2014submodular, nemhauser1978analysis, calinescu2011maximizing, bach2013learning}.  Submodular functions naturally model notions of diversity, representativeness, and information coverage, and thus appear in problems such as sensor placement~\cite{krause2008near}, data summarization~\cite{lin2011cl
ass}, influence maximization~\cite{kempe2003maximizing}, and active learning~\cite{golovin2011adaptive}.  
\begin{figure}[t]
\centering
    \includegraphics[scale=0.23]{Fig/schem.png}
\caption{{\small Spatial comparison of the early-commitment effect in a 2D sensor placement task. The objective is to select deployment points (solid circles) from candidates (red $\times$) to cover a clustered data distribution (blue dots) under partition-matroid constraints (colored ellipses). (i) Sequential Greedy: The algorithm's discrete, myopic selection leads the first agent to choose a central "median" point to maximize immediate marginal gain, resulting in a locally optimal but globally suboptimal arrangement that fails to capture the four distinct clusters. (ii) Continuous Greedy: By maintaining a fractional representation that evolves along a continuous ascent trajectory, the agents avoid premature commitment. This allows them to "revisit" decisions implicitly and settle on a superior arrangement that accurately partitions and covers the true data distribution.}}
    \label{fig:forward_gradiant}
\end{figure}
A particularly important class of problems arises when element selection is restricted by a \emph{matroid constraint}, which generalizes independence structures such as cardinality, partition, or budget limits~\cite{calinescu2011maximizing}. The canonical formulation with a utility function $f:2^\mathcal{P}\to\mathbb{R}_{+}$ is
\begin{equation}\label{eq::canonical_prob}
\max_{\mathcal{S} \in \mathcal{I}} f(\mathcal{S}),
\end{equation}
where $\mathcal{I}$ denotes the independent sets of a matroid on the ground set $\mathcal{P}$. This problem is known to be NP-hard.

The celebrated classical  polynomial-time suboptimal solution to~\eqref{eq::canonical_prob} is the \emph{Sequential Greedy (SG)} algorithm~\cite{nemhauser1978analysis,fisher2009analysis}, which starting from empty set iteratively adds the element that provides the largest marginal gain in $f(\mathcal{S})$. Despite its simplicity and scalability, SG achieves only a $(1/2)$-approximation for monotone submodular functions under general matroid constraints. The continuous counterpart, the \emph{Continuous Greedy (CG)} algorithm~\cite{calinescu2011maximizing}, bridges this gap by optimizing over the \emph{multilinear extension} of $F$,
$$
F(x) = \mathbb{E}[f(\mathcal{R}(x))],
$$
where $\mathcal{R}(x)$, $x\in[0,1]^{|\mathcal{P}|}$, is a random subset including each element $i$ of ground set $\mathcal{P}$ independently with probability $x_i\in[0,1]$. By following a continuous ascent trajectory within the matroid polytope and integrating infinitesimal greedy steps, CG achieves the optimal $(1-1/e)$ approximation guarantee where final solution is obtained by loss-less rounding procedure. Intuitively, while SG makes irrevocable discrete selections in its discrete, myopic selection, CG maintains a fractional representation of the solution that gradually evolves toward a balanced allocation of probabilities across competing elements, thereby mitigating the early-commitment effect inherent to SG. The qualitative impact of the early-commitment effect is visualized in Fig.~\ref{fig:forward_gradiant}, which demonstrates how the Sequential Greedy algorithm's irrevocable discrete choices lead to poor spatial coverage of clustered data compared to the balanced allocation achieved by Continuous Greedy.

Despite its theoretical elegance and improved optimality gap, deploying CG, especially in distributed or networked systems introduces significant computational and communication challenges. Each iteration requires evaluating or estimating the gradient $\nabla F(x)$, which depends on the contribution of all elements of the ground set $\mathcal{P}$, which can be distributed among the agents across the network, as in partition matroid case. In decentralized settings, this implies that every agent must exchange information about the local elements for which its local copy of $x$ is non-zero. Consequently, the distributed realization of CG (e.g.,~\cite{AM-HH-AK:18,rezazadeh2023distributed}) involves not only the local consensus of the decision vector $x$ among neighboring agents but also the exchange of gradient-related statistics and local ground set embeddings across the network. Such requirements lead to substantial communication overhead and latency. 

This work proposes a methodology to decrease the communication overhead of CG in distributed setting. We demonstrate this method over a server-assisted distributed implementation 
of the continuous greedy algorithm under a partition-matroid structure, 
where each agent maintains and updates a local block of the decision 
vector $x$ and relies on a central server to aggregate and 
broadcast the information needed for global gradient estimation. Communication overhead in this architecture arises from two coupled 
sources: (\textit{i}) each agent must share its local block of $\mathbf{x}_i$ with the server so that all agents operate on a consistent global state when estimating the gradient $\nabla F(x)$, and (\textit{ii}) whenever a component of $x_i$ becomes non-zero---indicating that the corresponding element has been activated---the agent must also transmit the associated data point 
to the server for redistribution to other agents. Both transmissions 
are necessary for accurate gradient computation across the network, and their combined frequency directly determines the communication overhead of the system. While other distributed topologies could 
naturally benefit from the proposed thresholding framework, we limit the scope of this work to the server-assisted setting as a principled first step toward communication-efficient distributed submodular 
optimization. Our proposed method can be extended to other distributed settings such as those in~\cite{AM-HH-AK:18,rezazadeh2023distributed} over communication graphs.





Motivated by these limitations, we propose \texttt{CG-$\eta$-Online}, 
a threshold-based variant of the continuous greedy algorithm designed 
to reduce computational and communication overhead in large-scale and 
decentralized settings. The key idea is to allow each agent to 
selectively restrict its gradient evaluations to a small subset of 
candidate elements, expanding this subset only when a local progress 
indicator signals insufficient coverage of the full candidate block. 
This selective activation mechanism preserves the near-optimality of 
continuous greedy while substantially reducing the number of gradient 
evaluations and the volume of information exchanged across agents. 


\emph{Related work}: There is a rich body of work in optimization and signal processing that uses \emph{thresholding} or \emph{hard-threshold} operators. For example, the compressed sensing literature has developed \emph{iterative hard thresholding}~(IHT) and its variants to enforce sparsity constraints~\cite{pan2017convergent, yuan2014gradient, foucart2011hard}, and other works consider constrained thresholded updates in nonconvex 
optimization~\cite{liu2020between}. While superficially similar in name, our thresholding mechanism differs fundamentally in both goals and operation. Specifically,~\cite{pan2017convergent} targets sparsity-constrained 
minimization via Armijo-type step sizes and support selection 
updates;~\cite{yuan2014gradient} combines gradient steps with thresholded projection onto candidate support sets for structured sparse recovery; and~\cite{foucart2011hard} selects signal support under linear measurement models in compressive sensing. In~\cite{liu2020between}, thresholding alternates with gradient descent to optimally balance convergence stability 
and sparsity enforcement in continuous optimization. In contrast, \texttt{CG-$\eta$-Online} employs thresholding not to enforce sparsity, but to \emph{adaptively decide when to expand} the active set for  gradient evaluation. Our $\eta$-threshold rule is guided by a ratio of  marginal gains, operates blockwise under a partition matroid structure, and  is motivated by reducing communication overhead in distributed submodular 
optimization---rather than minimizing a continuous objective with sparsity constraints.

Beyond the thresholding literature, scalability in submodular optimization has also been pursued through two complementary lines of work: acceleration within the discrete greedy framework and distributed partition-and-merge strategies. Two prominent lines of work address scalability in submodular maximization from complementary directions. \emph{Lazy greedy}~\cite{minoux1978accelerated, 
leskovec2007cost} accelerates the Sequential Greedy (SG) algorithm by exploiting the diminishing-returns property to skip marginal gain evaluations via cached upper bounds, thereby reducing function queries without altering the selection logic. While effective in the discrete setting, lazy greedy inherits the $(1/2)$-approximation ceiling of SG and does not extend 
naturally to the continuous domain or address communication overhead in distributed implementations. MapReduce-based approaches~\cite{mirzasoleiman2013distributed, 
kumar2015fast} achieve communication efficiency through a partition-and-merge paradigm: each machine runs a local greedy pass on its data shard, and the 
results are aggregated in a single communication round. Although this reduces inter-machine coordination, the partition-and-merge strategy incurs an approximation loss---typically yielding a $(1/4)$-approximation or 
worse---due to the lack of global coordination during local selection. In contrast, \texttt{CG-$\eta$-Online} operates entirely within the continuous 
greedy framework and preserves the optimal $(1-1/e)$-approximation guarantee. 
Rather than partitioning computation across machines or caching upper bounds, 
it reduces gradient evaluations and communication overhead through an 
adaptive $\eta$-threshold rule that governs when each agent must expand its 
active set, achieving communication efficiency without sacrificing 
near-optimality.



\emph{Statement of  contributions}: Our proposed  thresholding policy yields a new class of continuous greedy algorithms. Unlike static or pre-defined truncation schemes, the proposed approach dynamically expands active sets based on local progress indicators, ensuring that gradient and communication efforts are directed toward the most informative elements. The motivation behind this design is to reduce the communication overhead inherent in distributed submodular optimization, where transmitting local element information or gradient statistics can be costly. The \texttt{CG-$\eta$-Online} algorithm retains the monotone ascent property of continuous greedy dynamics while adaptively regulating which agents or coordinates become active through an $\eta$-thresholding rule. 

In summary, this paper introduces a threshold-driven mechanism for submodular maximization under partition-matroid constraints, bridging the gap between theoretical optimality and communication efficiency. The main contributions are:
\begin{itemize}
    \item A novel threshold-based continuous greedy algorithm that adaptively expands active sets based on per-agent progress indicators;
    \item Theoretical analysis establishing approximation guarantees that incorporate both threshold parameters and function curvature;
    \item Empirical validation demonstrating favorable trade-offs between solution quality and computational efficiency.
\end{itemize}


==> intro_reza.tex <==
\section{Introduction}

Submodular maximization has emerged as a cornerstone of modern discrete and combinatorial optimization, underpinning a wide range of applications in machine learning, control, and networked decision-making~\cite{krause2014submodular, nemhauser1978analysis, calinescu2011maximizing, bach2013learning}. A set function $F: 2^{\mathcal{V}} \to \mathbb{R}_{+}$ defined on a finite ground set $\mathcal{V}$ is called \emph{submodular} if it satisfies the diminishing-returns property
\begin{align*}
F(A \cup \{e\}) - F(A) \ge F(B \cup \{e\}) - F(B), \\
\quad \forall A \subseteq B \subseteq \mathcal{V},\ e \notin B.
\end{align*}
This property captures the intuitive principle that the marginal gain of adding an element decreases as the context set grows. Submodular functions naturally model notions of diversity, representativeness, and information coverage, and thus appear in problems such as sensor placement~\cite{krause2008near}, data summarization~\cite{lin2011class}, influence maximization~\cite{kempe2003maximizing}, and active learning~\cite{golovin2011adaptive}.  




\begin{figure}[t]
\centering
    \includegraphics[scale=0.28]{Fig/schem.png}
\caption{{\small Comparison between \textit{Sequential Greedy} and \textit{Continuous Greedy} algorithms in a 2D sensor placement task. 
    Each colored ellipse represents the decision region of a deploying agent, red ``$\times$'' marks indicate candidate locations, 
    and colored circles denote the chosen deployment locations. The blue points correspond to the underlying data distribution.}}\vspace{-0.1in}
    \label{fig:forward_gradiant}
\end{figure}


A particularly important class of problems arises when element selection is restricted by a \emph{matroid constraint}, which generalizes independence structures such as cardinality, partition, or budget limits~\cite{calinescu2011maximizing,schrijver2003combinatorial}. The canonical formulation is
\begin{equation} \label{main:prob:eq}
\max_{S \in \mathcal{I}} F(S),
\end{equation}
where $\mathcal{I}$ denotes the family of independent sets of a matroid defined on the ground set $\mathcal{V}$. A classical algorithm for this problem is the \emph{Sequential Greedy (SG)} method~\cite{nemhauser1978analysis,fisher2009analysis}, which iteratively selects the element that yields the largest marginal gain with respect to the current set. Owing to its simplicity and computational efficiency, SG has become a widely used baseline for large-scale submodular optimization. However, under general matroid constraints the algorithm guarantees only a $(1/2)$-approximation for monotone submodular functions. This limitation arises from the inherently \emph{irreversible} nature of sequential greedy selections, i.e., once an element is selected, the choice cannot be revised, which may lead to suboptimal configurations when early selections restrict future possibilities.

The \emph{Continuous Greedy (CG)} algorithm~\cite{calinescu2011maximizing} addresses this limitation by optimizing the \emph{multilinear extension} of the submodular function,
\[
f(x) = \mathbb{E}[F(R(x))],
\]
where $R(x)$ is a random subset that includes each element $i$ independently with probability $x_i$. Instead of committing to discrete selections, CG maintains a fractional vector $x$ that evolves continuously inside the matroid polytope. At each step the algorithm follows a direction that maximizes the inner product with the gradient $\nabla f(x)$, gradually increasing the probability mass assigned to promising elements. By integrating these infinitesimal greedy steps over time, continuous greedy achieves the optimal $(1-1/e)$ approximation guarantee for monotone submodular maximization under matroid constraints~\cite{calinescu2011maximizing}.

Intuitively, while SG commits to elements sequentially and irrevocably, CG maintains a soft allocation of selection probabilities across all candidates, allowing the algorithm to adaptively balance competing elements before producing a final discrete solution via rounding. This distinction is illustrated in Fig.~\ref{fig:forward_gradiant}. In the depicted sensor placement example, sequential greedy commits early to a central location that appears locally beneficial but ultimately limits coverage of the surrounding clusters. In contrast, continuous greedy maintains a fractional representation during the optimization process, allowing the algorithm to better distribute sensing locations across the underlying data structure and thereby achieve a higher-quality configuration.


Despite its strong theoretical guarantees, deploying CG algorithm in distributed or networked environments presents significant computational and communication challenges. Each iteration requires estimating the gradient of the multilinear extension, $\nabla f(x)$, whose coordinates correspond to the expected marginal gains of individual elements in the ground set $\mathcal{V}$. Consequently, evaluating this gradient typically involves computing marginal contributions across all candidate elements.

In decentralized settings, where the ground set is partitioned across multiple agents, this process requires aggregating marginal-gain information across the network. Each agent must therefore communicate statistics associated with its local elements while simultaneously maintaining consensus on the shared decision vector $x$. As a result, distributed implementations of CG require both coordination of the decision variables and repeated exchange of gradient-related information among agents. These operations can introduce substantial communication overhead and latency, particularly when the ground set $\mathcal{V}$ is large~\cite{rezazadeh2023distributed}.

Motivated by these limitations, we seek to design a variant of the continuous greedy algorithm that better aligns with distributed environments by reducing the number of coordinates that actively participate in the update process. While the algorithm we develop in this work is presented in a centralized form, its structure is specifically designed to facilitate decentralized implementations. To this end, we introduce a threshold-based continuous greedy variant, \underline{A}daptive \underline{T}hresholded \underline{C}ontinuous \underline{G}reedy (\textit{ATCG}) which adaptively regulates a dynamically expanding subset of candidate elements. The key idea is to maintain, for each block or agent $i$, a small \emph{active set} $A_i$ of candidates that participate in the restricted greedy update. A scalar \emph{progress ratio} $\eta_i$ measures how well the best candidate currently contained in the active set approximates the best candidate in the full block $B_i$:
\[
\eta_i =
\frac{\max_{j \in A_i} [\nabla f(\vect{x})]_{(i,j)}}
{\max_{j \in B_i} [\nabla f(\vect{x})]_{(i,j)}} .
\]

When $\eta_i$ remains above a predefined threshold $\tau$, the algorithm continues operating within the existing active set. Only when $\eta_i$ falls below $\tau$ is a new promising element added to $A_i$. In this way, the method adaptively determines when additional gradient information is necessary and when the current candidate set remains sufficiently representative. This structure naturally lends itself to distributed realizations in which only active elements participate in gradient aggregation and communication. As a result, the communication burden scales with the size of the active sets rather than the full ground set, providing a pathway toward more communication-efficient implementations of continuous greedy methods.

There is a rich body of work in optimization and signal processing that uses \emph{thresholding} or \emph{hard-threshold} operators. For example, the compressed sensing literature has developed \emph{iterative hard thresholding} (IHT) and its variants to enforce sparsity constraints~\cite{pan2017convergent, yuan2014gradient, foucart2011hard}, and other works consider constrained thresholded updates in nonconvex optimization~\cite{liu2020between}. While superficially similar in spirit, our thresholding mechanism is fundamentally different in goals and operation.

Authors in~\cite{pan2017convergent} present a \emph{Convergent Iterative Hard Thresholding} method for nonnegative sparse optimization, employing an Armijo-type step size and support selection updates. That work targets sparsity-constrained minimization problems in continuous domains, not combinatorial subset selection. In ~\cite{yuan2014gradient} authors analyze a \emph{Gradient Hard Thresholding Pursuit} method (GHTP) for structured sparse recovery, combining gradient steps with thresholded projection onto candidate support sets. Their thresholding is used to enforce sparsity per iteration, whereas ours governs when to expand active gradient sets. ~\cite{foucart2011hard} discusses the theoretical behavior of the Hard Thresholding Pursuit (HTP) algorithm in compressed sensing frameworks. Their thresholding focuses on selecting signal support under linear measurement models, rather than submodular objective increments. In~\cite{liu2020between}, authors analyze a family of iterative thresholding algorithms that alternate between gradient descent and thresholding steps for sparse-constrained optimization. Their goal is to identify thresholding operators that optimally balance convergence stability and sparsity enforcement. Unlike our approach, their thresholding acts as a projection operator enforcing sparsity in continuous optimization, whereas our $\tau$-thresholding policy dynamically governs when to expand active gradient sets in submodular maximization, motivated by communication efficiency rather than sparsity constraints.




In contrast to prior thresholding methods developed in the context of constrained optimization, our \textit{ATCG} algorithm employs thresholding not to enforce sparsity, but to \emph{adaptively decide when to expand} the active set for gradient evaluation. Unlike these existing approaches, our thresholding rule is guided by a ratio of marginal gains ($\eta_i$), operates in a blockwise manner under a partition matroid structure, and is primarily motivated by the goal of reducing communication overhead in prospective distributed extensions of submodular optimization, rather than minimizing a continuous objective with sparsity constraints.

\textbf{Novelty and contributions.}
This work introduces a threshold-driven variant of the continuous greedy algorithm, named \textit{ATCG}, designed to regulate which candidate elements actively participate in the greedy updates. Unlike classical continuous greedy implementations that repeatedly evaluate marginal gains over the entire ground set, \textit{ATCG} maintains dynamically expanding \emph{active sets} whose growth is controlled by a blockwise progress indicator. This mechanism allows the algorithm to adaptively focus computation on the most informative elements while preserving the ascent structure of continuous greedy dynamics. Although the algorithm is developed and analyzed in a centralized setting, its design is motivated by communication bottlenecks that arise in distributed implementations of submodular maximization. In particular, by regulating which coordinates remain active during the optimization process, \textit{ATCG} provides a natural framework for limiting the number of elements that would participate in gradient aggregation and communication in decentralized environments.

% The main contributions of this work are summarized as follows:

% \begin{itemize}
% \item We introduce \textit{Adaptive Thresholded Continuous Greedy (\textit{ATCG})}, a threshold-driven continuous greedy algorithm that adaptively expands blockwise active sets using a progress ratio that compares the best candidate in the active set to the best candidate in the full block.

% \item We show how the proposed thresholding mechanism regulates participation of candidate elements in the greedy update, providing a structured way to control which coordinates remain active during optimization.

% \item We demonstrate that the resulting algorithm preserves the monotone ascent behavior of continuous greedy dynamics while introducing an adaptive mechanism that is naturally compatible with distributed implementations.

% \item Empirical studies on class-balanced image prototype selection under partition-matroid constraints demonstrate that \textit{ATCG} achieves a favorable trade-off between solution quality and computational scalability.
% \end{itemize}


==> intro_v3.tex <==
\section{Introduction}

Submodular maximization has emerged as a cornerstone of modern discrete 
and combinatorial optimization, with relevance to a wide range of applications 
in machine learning, control, and networked decision-making~\cite{krause2014submodular, 
nemhauser1978analysis, calinescu2011maximizing, bach2013learning}. 
Submodular functions naturally model notions of diversity, 
representativeness, and information coverage, and thus appear in problems 
such as sensor placement~\cite{krause2008near}, data 
summarization~\cite{lin2011class}, influence maximization~\cite{kempe2003maximizing}, 
and active learning~\cite{golovin2011adaptive}.

\begin{figure}[t]
\centering
    \includegraphics[scale=0.23]{Fig/schem3.png}
\caption{{\small 
Illustration of the early-commitment effect of SG 
(left) and its mitigation via CG (right) in a 2D sensor placement 
task. Deployment points (solid circles) are selected from candidates 
(red~$\times$) to cover a clustered data distribution (blue dots) 
under partition-matroid constraints, where each colored region 
represents the candidate set of the corresponding agent.}}
    \label{fig:forward_gradiant}
\end{figure}

A central problem in this area is constrained submodular maximization 
under a \emph{matroid constraint}, which generalizes independence 
structures such as cardinality, partition, or budget 
limits~\cite{calinescu2011maximizing}. The canonical formulation with 
utility function $f:2^\mathcal{P}\to\mathbb{R}_{+}$ is
\begin{equation}\label{eq::canonical_prob}
\max_{\mathcal{S} \in \mathcal{I}} f(\mathcal{S}),
\end{equation}
where $\mathcal{I}$ denotes the independent sets of a matroid on ground 
set $\mathcal{P}$. This problem is NP-hard. 

The celebrated \emph{Sequential Greedy (SG)} algorithm~\cite{nemhauser1978analysis, 
fisher2009analysis} offers a classical polynomial-time solution by 
iteratively selecting the element with the largest marginal gain in 
$f(\mathcal{S})$, starting from the empty set. Despite its simplicity 
and scalability, SG achieves only a $(1/2)$-approximation for monotone 
submodular functions under general matroid constraints. This limitation 
arises from the inherently \emph{irreversible} nature of greedy 
selections, i.e., once an element is chosen, the decision cannot be revised, 
which can lead to suboptimal configurations when early selections 
restrict future possibilities. The \emph{Continuous Greedy (CG)} 
algorithm~\cite{calinescu2011maximizing} closes this gap by optimizing 
over the \emph{multilinear extension} of $f$,
\begin{align}\label{eq::multi_linear}
F(\vect{x}) =& \mathbb{E}[f(\mathcal{R}(\vect{x}))]\nonumber\\
&~\sum_{\mathcal{R} \subset \mathcal{P}}{}\! \!f(\mathcal{R})\! \prod_{p \in \mathcal{R}}^{}\!\! [\vect{x}]_p \prod_{p \not\in \mathcal{R}}^{}\!(1-[\vect{x}]_p),
\end{align}
where $\vect{x}\in[0,1]^{|\mathcal{P}|}$ is the \emph{probability membership vector}, and $\mathcal{R}(\mathbf{x})$ includes each 
element $p$ independently with probability $[\vect{x}]_p\in[0,1]$. Instead of committing 
to discrete selections, CG maintains a fractional vector $\vect{x}$ that 
evolves continuously within the matroid polytope, at each step following 
a direction that maximizes the inner product with the gradient 
$\nabla F(\vect{x})$ and gradually increasing the probability mass assigned to 
promising elements. By integrating these infinitesimal greedy steps, CG 
achieves the optimal $(1-1/e)$ approximation, with the final solution 
recovered via a lossless rounding step. 

The qualitative difference between SG and CG is illustrated 
in Fig.~\ref{fig:forward_gradiant}: SG's early commitment 
to a central median point fails to capture the four distinct 
data clusters, while CG's deferred, fractional allocation 
produces a superior arrangement. Tightening the optimality 
gap directly translates to cost savings and efficiency gains 
across domains such as sensor scheduling, logistics, and 
robotic coverage.

Despite its theoretical elegance and improved approximation guarantee, 
deploying CG in distributed or networked systems introduces significant 
computational and communication challenges. Each iteration requires 
evaluating or estimating the gradient $\nabla F(\vect{x})$, which depends on 
the contribution of all elements of the ground set $\mathcal{P}$---distributed 
among agents across the network, as in the partition matroid case. 
Critically, since CG operates over the multilinear extension, the 
probability membership  vector $\vect{x}$ evolves continuously and its components gradually 
become non-zero over the course of the algorithm. Each non-zero 
component $[\mathbf{x}(t)]_j > 0$ signifies that element $j$ is 
actively contributing to the gradient estimation, and every agent 
requires the feature embedding of that element to compute $\nabla F(\vect{x})$ 
globally. As $\vect{x}$ tends to become dense throughout the CG trajectory, 
this effectively forces agents to exchange the feature data of nearly 
every element in the ground set which is resulting in a communication burden 
that scales with $|\mathcal{P}|$ rather than the size of any local 
selection. This stands in sharp contrast to SG, where each agent need 
only broadcast its single final selected element upon termination, 
incurring a one-time, minimal data transmission at the price of a 
suboptimal $(1/2)$-approximation~guarantee.

\emph{Statement of contribution}: To address this overhead, we propose 
\textit{ATCG} (\underline{A}daptive \underline{T}hresholded 
\underline{C}ontinuous \underline{G}reedy), a threshold-based variant 
of CG demonstrated in a server-assisted distributed setting under a 
partition-matroid structure, where each agent maintains a local partition of the ground set and local partition 
of the probability membership vector $\vect{x}$ and relies on a central server for gradient 
aggregation. Each agent selectively restricts gradient evaluations to 
a small, dynamically expanding active subset, triggering expansion 
only when the ratio of the best marginal gain within the active subset 
to that of the full partition falls below a predefined threshold 
$\tau$---the ``Adaptive'' in the name reflects this 
iteration-by-iteration expansion rule, in contrast to static or 
pre-defined truncation schemes. Since only active elements contribute 
non-zero entries to $\vect{x}$, this directly limits the volume of feature 
data exchanged between agents and the server, keeping communication 
overhead proportional to the active set size rather than 
$|\mathcal{P}|$. Theoretical analysis establishes that the coverage 
factor $\tau_{\mathrm{eff}} = \max\{\tau, 1-c\}$, jointly determined by the 
threshold parameter and the function curvature, interpolates between a threshold-controlled guarantee and a low-curvature regime where \textit{ATCG} approaches the performance of CG.
Experiments on image summarization and prototype selection demonstrate that \textit{ATCG} matches the solution quality of full CG while significantly reducing communication to the server.


\emph{Related work}: Thresholding and hard-threshold operators have a 
rich history in optimization and signal processing. The compressed 
sensing literature has developed \emph{iterative hard thresholding} 
(IHT) and its variants to enforce sparsity constraints~\cite{pan2017convergent, 
yuan2014gradient, foucart2011hard}, and related works apply constrained 
thresholded updates in nonconvex optimization~\cite{liu2020between}. 
While superficially similar in name, our mechanism differs fundamentally 
in both goal and operation. The work in \cite{pan2017convergent} targets 
sparsity-constrained minimization via Armijo-type step sizes; 
\cite{yuan2014gradient} enforces sparsity per iteration via thresholded 
projection onto candidate support sets; \cite{foucart2011hard} selects 
signal support under linear measurement models; and \cite{liu2020between} 
alternates thresholding with gradient descent to balance convergence 
stability and sparsity. In contrast, \textit{ATCG} uses 
thresholding not to enforce sparsity, but to \emph{adaptively decide 
when to expand} the active set for gradient evaluation which is guided by a 
ratio of marginal gains, operating prtition-wise under a partition matroid, 
and motivated by communication efficiency rather than sparse 
minimization.

Scalability in submodular optimization has also been pursued through 
two complementary directions. \emph{Lazy greedy}~\cite{minoux1978accelerated},\cite{mirzasoleiman2015lazier} accelerates SG by caching marginal gain upper bounds 
to skip redundant evaluations, but inherits the $(1/2)$-approximation 
ceiling of SG and does not extend to the continuous domain. 
MapReduce-based approaches~\cite{mirzasoleiman2013distributed, 
kumar2015fast} achieve one-round communication efficiency through a 
partition-and-merge paradigm, but incur approximation loss---typically 
$(1/4)$ or worse---due to the absence of global coordination during 
local selection. \textit{ATCG} operates entirely within the 
CG framework, preserving the $(1-1/e)$ guarantee while achieving 
communication efficiency through an adaptive $\tau$-threshold rule, 
without partitioning computation or sacrificing near-optimality.

\begin{comment}
\emph{Statement of contributions}: This paper introduces 
\textit{ATCG} (Adaptive Thresholded Continuous Greedy), a 
threshold-driven variant of continuous greedy that bridges 
theoretical optimality and communication efficiency under 
partition-matroid constraints. Unlike classical CG implementations 
that activate---and therefore require data exchange for---every 
element in the ground set as $x$ becomes dense, \textit{ATCG} 
maintains dynamically expanding active sets whose growth is governed 
by a blockwise progress indicator, keeping communication overhead 
proportional to the active set size rather than $|\mathcal{P}|$ 
throughout the optimization trajectory. Notably, the approximation 
guarantee of \textit{ATCG} gracefully interpolates between the 
$(1/2)$-approximation of SG and the $(1-1/e)$ guarantee of CG, 
with the threshold parameter $\eta$ and the function curvature 
jointly determining the effective coverage factor. The main 
contributions are:
\begin{itemize}
    \item A novel threshold-based continuous greedy algorithm that 
    adaptively expands active sets based on per-agent progress 
    indicators, directly limiting inter-agent feature data exchange;
    \item Theoretical analysis establishing approximation guarantees 
    that incorporate both threshold parameters and function 
    curvature, with the coverage factor $\alpha = \max\{\eta, 1-c\}$ 
    interpolating between the efficiency of SG and the near-optimality 
    of CG;
    \item Empirical validation on image summarization and prototype 
    selection tasks demonstrating that moderate threshold values 
    $\eta \in [0.7, 0.9]$ preserve $95\%$--$99\%$ of full CG 
    solution quality while reducing gradient evaluations by 
    $40\%$--$60\%$.
\end{itemize}
\end{comment}

==> numerical_example_origional.tex <==
\section{Numerical Evaluation}\label{numerical}
To illustrate the practical motivation behind \textit{ATCG}, we consider a networked robotic sensing scenario built on a subset of the CIFAR-10 dataset containing visually related animal categories, such as deer, frog, bird, horse, cat, and dog. In this interpretation, a team of robots monitors an environment populated by these animal types, and each robot is assigned responsibility for one category. The task of each robot is to select a representative prototype from its local candidate set, while the team collectively aims to choose one prototype per category so that the selected set provides the best overall coverage of the environment. We model this task as a class-balanced prototype selection problem under a partition matroid constraint with $\kappa_i=1$, where each partition corresponds to the candidate images associated with one category. Let $\mathcal{V}=\bigcup_{i=1}^N B_i$ denote the partitioned ground set, and let
\[
\mathcal{I}
=
\{S\subseteq \mathcal{V}\mid |S\cap B_i|\le 1,\ \forall i=1,\dots,N\}
\]
be the feasible family. Each image is first embedded into a feature space using a pretrained convolutional neural network (ResNet), and pairwise similarities are then computed from these feature embeddings through an RBF kernel
$
K(p,q)=\exp\!\left(-\frac{\|z_p-z_q\|_2^2}{2\sigma^2}\right).
$
The global utility is then defined by the facility-location objective
\[
f(S)=\sum_{p\in\mathcal{V}} \max_{q\in S} K(p,q),
\]
and the resulting optimization problem is \eqref{main:prob:eq}. A key feature of this setup is that the decisions of different partitions are coupled through the global facility-location objective. Since animal categories such as deer, horse, cat, and dog exhibit similar visual structure, their embeddings often have non-negligible cross-class similarity under the RBF kernel. Consequently, the prototype selected by one partition may already cover images that would otherwise be represented by another partition. This coupling effect is illustrated in Fig.~\ref{fig:rbf_cifar_coupling}, which reports the inter-class mean RBF similarity matrix for the CIFAR animal subset.


\begin{figure}[t]
\centering
    \includegraphics[scale=0.33]{Fig/tau1_trajectory.png}
\caption{\small Facility-location objective trajectory for CG and \textit{ATCG} with $\tau=0.30$ on the CIFAR animal subset. The results show that \textit{ATCG} closely tracks the performance of CG while using a thresholded active-set update rule.}
\label{fig:traj_cifar_atcg}
\end{figure}


\begin{figure}[t]
\centering
    \includegraphics[scale=0.33]{Fig/tau1_comm_cumulative.png}
\caption{\small Cumulative communication to the server for CG and \textit{ATCG}. The results show that \textit{ATCG} substantially reduces the communication load while maintaining performance comparable to CG.}
\label{fig:comm_cifar_atcg}
\end{figure}

Although \textit{ATCG} is developed and analyzed in a centralized setting, this example admits a natural distributed interpretation. We assume that a global dataset describing the environment is available at a central server, and that each robot can query an oracle to obtain the marginal gains required for gradient computation. Because the gradient of the multilinear extension depends on the globally selected prototypes, each robot must communicate newly activated candidate images to the server so that subsequent marginal gains can be updated consistently. In this interpretation, communication cost is measured by the number of new candidate images transmitted to the server during the optimization.



The results further highlight the practical advantage of \textit{ATCG}. As shown in Fig.~\ref{fig:traj_cifar_atcg}, \textit{ATCG} closely tracks the objective trajectory of the full continuous greedy method, showing that the thresholded active-set rule preserves solution quality. After rounding the fractional solution $\vect{x}$ to a feasible discrete set via partition-wise argmax rounding, the resulting set-function values are $144.89$ for CG and $143.63$ for \textit{ATCG}. At the same time, Fig.~\ref{fig:comm_cifar_atcg} shows that \textit{ATCG} substantially reduces cumulative communication to the server compared to CG. This behavior is closely explained by the active-set evolution in Fig.~\ref{fig:active_growth_cifar_atcg}. In the early iterations, \textit{ATCG} has not yet explored enough candidates, so the active sets expand more aggressively. After sufficient informative elements have been identified, however, the active sets satisfy the $\tau$-threshold condition and no longer need to grow significantly. In particular, from roughly iteration 50 onward, the active-set size remains essentially unchanged, which is consistent with the communication curve in Fig.~\ref{fig:comm_cifar_atcg}, where no further communication is added to the server during the later iterations. This clearly demonstrates the main benefit of \textit{ATCG} which is once a sufficiently informative active set has been formed, the method continues optimizing while avoiding unnecessary communication overhead.


% \begin{figure}[t]
% \centering
%     \includegraphics[scale=0.28]{Fig/fig_atcg_rbf_heatmap.png}
% \caption{\small Inter-class mean RBF similarity matrix for the CIFAR animal subset, showcasing the coupling effect between the animal images.}\vspace{-0.1in}
%     \label{fig:rbf_cifar_coupling}
% \end{figure}


% \begin{figure}[t]
% \centering
%     \includegraphics[scale=0.33]{Fig/tau1_trajectory.png}
% \caption{\small Facility-location objective trajectory for CG and \textit{ATCG} with $\tau=0.30$ on the CIFAR animal subset. The results show that \textit{ATCG} closely tracks the performance of CG while using a thresholded active-set update rule.}
% \label{fig:traj_cifar_atcg}
% \end{figure}




% \begin{figure}[t]
% \centering
%     \includegraphics[scale=0.33]{Fig/tau1_comm_cumulative.png}
% \caption{\small Cumulative communication to the server for CG and \textit{ATCG}. The results show that \textit{ATCG} substantially reduces the communication load while maintaining performance comparable to CG.}
% \label{fig:comm_cifar_atcg}
% \end{figure}

\begin{figure}[t]
\centering
    \includegraphics[scale=0.33]{Fig/tau1_active_growth.png}
\caption{\small Growth of the total active-set size \(\sum_i |A_i|\) for \textit{ATCG}. The active sets expand only when needed and stabilize after a small number of iterations.}
\label{fig:active_growth_cifar_atcg}
\end{figure}





==> numerical_example_v1.tex <==
\section{Numerical Evaluation}\label{numerical}


{\color{red}
Consider a team of $N$ robots deployed to survey an unknown environment.
Each robot $i$ independently collects a local dataset $\mathcal{P}_i$ of
observations---images captured from its assigned region---and the union
$\mathcal{P} = \bigcup_{i=1}^N \mathcal{P}_i$ represents all collected data.
After data collection, each robot must identify which single observation from
$\mathcal{P}_i$ is most representative of the broader environment: this chosen
observation becomes the element that robot $i$ focuses on, while the union of
all selected observations should collectively provide the best possible coverage
of $\mathcal{P}$. To evaluate how representative any candidate observation is,
each robot compares it against a central repository of reference embeddings held
at the server---for example, a pretrained image database---which provides a
measure of how well the candidate covers the broader data distribution.
Crucially, this is not $N$ independent local problems: because the robots survey
a shared environment, the observation selected by robot $i$ may already account
for data that would otherwise need to be covered by a neighboring robot, similar
to the case illustrated in Fig.~\ref{fig:forward_gradiant}. The team therefore
faces a coupled, global selection problem---precisely the structure captured by
the partition-matroid formulation~\eqref{eq::partion_matroid} with $\kappa_i=1$.

To instantiate this scenario using realistic data, we construct the ground set
$\mathcal{P}$ from a subset of the CIFAR-10 dataset containing six visually
related animal categories: deer, frog, bird, horse, cat, and dog. Each category
corresponds to one partition $\mathcal{P}_i$, representing the local observations
collected by robot $i$ in its assigned region of the environment. The
partition-matroid~\eqref{eq::partion_matroid} constraint enforces $\kappa_i = 1$,
so each robot selects exactly one representative image. Each image is embedded
into a feature space using a pretrained ResNet, and pairwise similarities are
computed via the RBF kernel
\[
  K(p,q) = \exp\!\left(-\frac{\|\mathbf{z}_p - \mathbf{z}_q\|_2^2}{2\sigma^2}\right).
\]
The global utility is the facility-location objective
\[
  f(\mathcal{S}) = \sum_{p \in \mathcal{P}} \max_{q \in \mathcal{S}} K(p,q),
\]
which is monotone submodular and measures how well the selected observations
collectively cover all data in $\mathcal{P}$; the resulting problem is
\eqref{eq::canonical_prob} with $\mathcal{I}$ given in~\eqref{eq::partion_matroid}.
The inter-class RBF similarity matrix (Fig.~\ref{fig:rbf_cifar_coupling}) confirms
non-negligible cross-partition similarity among visually related categories such as
deer, horse, cat, and dog, making the facility-location objective non-separable
across blocks. This is precisely the coupling structure for which \textit{ATCG}'s
globally coordinated active-set expansion is essential.
}





Under the server-assisted protocol of Section~\ref{sec::problem}, the server holds
the full feature repository, and each robot $i$ transmits the feature embedding of
any newly activated observation $j \in \mathcal{P}_i$---i.e., any $j$ for which
$[\mathbf{x}_i]_j$ becomes non-zero for the first time---so that subsequent
gradient estimates $\{[\nabla F(\mathbf{x})]_j\}_{j \in \mathcal{P}_i}$ account
for the globally selected representatives. Total communication cost is therefore
$\sum_{i=1}^{N}|\mathcal{A}_i|$ at termination.

\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{Fig/tau1_trajectory.png}
\caption{\small Facility-location objective $f$ vs.\ iteration for CG and
\textit{ATCG} ($\tau{=}0.30$) on the CIFAR animal subset. The two trajectories
are nearly indistinguishable throughout all $100$ iterations. After
partition-wise argmax rounding of the fractional solution $\mathbf{x}(1)$, the
discrete values are $144.89$ (CG) and $143.63$ (\textit{ATCG})---a gap below
$1\%$---confirming that the $\tau$-coverage condition~\eqref{eq:eta_def} is
sufficient to preserve solution quality, consistent with Theorem~III.1.}
\label{fig:traj_cifar_atcg}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{Fig/tau1_comm_cumulative.png}
\caption{\small Cumulative communication to the server for CG and \textit{ATCG}.
CG's curve rises steadily as $\mathbf{x}$ densifies and more feature embeddings
must be transmitted; \textit{ATCG}'s curve rises only during the early exploration
phase and becomes completely flat once all progress ratios satisfy
$\eta_i \geq \tau$~\eqref{eq:eta_def}, after which no further feature embeddings
are uploaded. The gap between the two curves at termination quantifies the
communication saving delivered by the active-set restriction.}
\label{fig:comm_cifar_atcg}
\end{figure}

\textbf{Objective quality (Fig.~\ref{fig:traj_cifar_atcg}).}
\textit{ATCG} closely tracks the objective trajectory of the full CG method
throughout the optimization, and the sub-$1\%$ gap in the final rounded solutions
validates the prediction of Theorem~III.1: restricting gradient evaluations to the
active sets $\{\mathcal{A}_i\}$ via the $\tau$-coverage rule~\eqref{eq:eta_def}
introduces only a controlled approximation loss relative to full CG. The
negligible practical gap relative to this bound is further consistent with the
curvature-aware guarantee of Theorem~III.2: the facility-location objective over
visually similar animal categories has low total curvature $c$, so the effective
rate $\max\{\tau,\,1{-}c\}$ substantially exceeds $\tau$ alone and
\textit{ATCG} approaches the classical $(1-e^{-1})$ bound of full CG.

\textbf{Communication reduction (Fig.~\ref{fig:comm_cifar_atcg}).}
In contrast to CG, whose communication grows steadily as $\mathbf{x}$ densifies,
\textit{ATCG}'s cumulative upload curve flattens well before the optimization
terminates. This is the direct signature of active-set stabilization: once every
$\eta_i \geq \tau$, the expansion rule in Algorithm~2 ceases to fire and no
further feature embeddings are transmitted to the server---yet the objective
continues to improve on the already-cached information, demonstrating that
$\sum_{i=1}^{N}|\mathcal{A}_i| \ll |\mathcal{P}|$ suffices for near-optimal
performance.

\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{Fig/tau1_active_growth.png}
\caption{\small Growth of the total active-set size $\sum_i|\mathcal{A}_i|$ for
\textit{ATCG}. Rapid growth in the early iterations (exploration phase, $\eta_i <
\tau$) gives way to a completely flat plateau from roughly iteration~$50$ onward
(exploitation phase, $\eta_i \geq \tau$ for all blocks), matching precisely the
communication cutoff visible in Fig.~\ref{fig:comm_cifar_atcg}. The final plateau
value $\sum_i|\mathcal{A}_i| \ll |\mathcal{P}|$ is the total number of feature
embeddings ever uploaded to the server.}
\label{fig:active_growth_cifar_atcg}
\end{figure}

\textbf{Active-set dynamics (Fig.~\ref{fig:active_growth_cifar_atcg}).}
Figure~\ref{fig:active_growth_cifar_atcg} makes the communication cutoff in
Fig.~\ref{fig:comm_cifar_atcg} mechanistically transparent. In the first
${\sim}50$ iterations, one or more blocks have $\eta_i < \tau$, so the expansion
step (Algorithm~2, line~11) fires and $\sum_i|\mathcal{A}_i|$ grows as new
candidates are admitted. Once enough informative observations are activated, all
blocks simultaneously satisfy $\eta_i \geq \tau$~\eqref{eq:eta_def} and the curve
levels off to a constant---exactly the flat region of the communication curve.
From this point onward, optimization proceeds entirely on locally cached embeddings
with zero additional uploads, demonstrating the central benefit of \textit{ATCG}:
the exploration phase pays a bounded, one-time communication cost to identify a
$\tau$-covering representative set, after which the exploitation phase drives the
objective to its final value at no further communication expense.

==> numerical_example_v2.tex <==
\section{Numerical Evaluation}\label{numerical}
We consider a target monitoring task involving a group of $N$ robots. Each robot is provided with a large, labeled image archive $\mathcal{D}$ consisting of images from $N$ target categories (e.g., $N$ distinct groups of animals). These archival images can be visualized as the blue data points in Fig.~\ref{fig:forward_gradiant} within a feature space where similar categories naturally form clusters, though some features may overlap. Each robot $i$ independently collects live target images from its patrol area, producing a local image set $\mathcal{P}_i$ (like the cross points in Fig.~\ref{fig:forward_gradiant})\footnote{In Fig.~\ref{fig:forward_gradiant}, the matroid constraint is a partition matroid, with non-overlapping local ground sets defined for each agent $i \in [N] = \{1, \dots, N\}$ as $\mathcal{P}_i = \{(i, b) \mid b \in \mathcal{B}_i\}$, where $\mathcal{B}_i$ represents the selection choices of agent $i$.}. The union $\mathcal{P} = \bigcup_{i=1}^{N} \mathcal{P}_i$ constitutes the full ground set of candidate images distributed across the team. 
Using the labeled archive as a reference, the team performs \emph{exemplar clustering}~\cite{krause2014submodular} so that each agent selects a representative target point from $\mathcal{P}_i$. Collectively, these choices are intended to form a set of $N$ data points that best characterize each target category so each agent can focus on one representation. An agent's choice directly impacts others; if one agent selects a specific representative to monitor, the other robots must focus on covering representatives from the remaining classes to ensure diverse coverage.


We instantiate this scenario on a subset of CIFAR-10 comprising six animal categories (deer, frog, bird, horse, cat, and dog). We randomly sample a subset of data from this dataset to construct the local set $\mathcal{P}_i$ of each agent. Images are embedded via a pretrained ResNet, and pairwise similarities are computed with the RBF kernel $K(p,q) = \exp(-\|\mathbf{z}_p - \mathbf{z}_q\|_2^2 / (2\sigma^2))$. The global utility is defined by the facility-location objective $f(\mathcal{S}) = \sum_{p \in \mathcal{P}} \max_{q \in \mathcal{S}} K(p,q)$ for any $\mathcal{S}\subseteq\mathcal{P}$, which is monotone submodular and measures how effectively the selected prototypes collectively cover all observed images in $\mathcal{P}$. The optimal multi-agent selection problem requires that $\mathcal{S}\in\mathcal{I}$, where $\mathcal{I}$ is the partition matroid defined in~\eqref{eq::partion_matroid}. The inter-class RBF similarity matrix (see \cite[Fig. 2]{rostami2026atcg}) confirms non-negligible cross-partition similarity among visually related categories such as deer, horse, cat, and dog. This coupling renders the objective non-separable across partitions, necessitating the globally coordinated active-set expansion of \textit{ATCG}. Under the server-assisted protocol of Section~\ref{sec:algo_theory}, the server
facilitates local active feature exchange and sharing aggregated global probability membership vector $\vect{x}$ among agents. %Robot~$i$ uploads the feature embedding of element $j \in \mathcal{P}_i$ only the first time $[\mathbf{x}_i]_j$ becomes non-zero. Total communication cost is $\sum_{i=1}^{N}|\mathcal{A}_i|$ at termination.

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[scale=0.3]{Fig/fig_atcg_rbf_heatmap.png}
\caption{\small Inter-class mean RBF similarity matrix for the CIFAR animal subset, illustrating the coupling effect between the animal images.}
\label{fig:rbf_cifar_coupling}
\end{figure}
\end{comment}


\begin{figure}[t]
\centering
\includegraphics[scale=0.3]{Fig/fig_tau_sweep_trajectory.png}
\caption{\reza{\small Objective trajectory \(F(\mathbf{x}_t)\) versus iteration for CG, SCG,
and \textit{ATCG} with different threshold values \(\tau\) on the CIFAR
animal subset. }}
\label{fig:traj_cifar_atcg}\vspace{-0.4in}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.3]{Fig/fig_tau_sweep_communication.png}
\caption{ \reza{\small Cumulative communication uploaded to the server for CG, SCG, and
\textit{ATCG} with different threshold values \(\tau\). %on the CIFAR animal subset.
} 
}
\label{fig:comm_cifar_atcg}\vspace{-0.1in}
\end{figure}


\textbf{Objective quality (Fig.~\ref{fig:traj_cifar_atcg})} \reza{shows that
\textit{ATCG} tracks CG throughout all \(100\) iterations without visible
deviation across the tested threshold values.} For \(\tau=0.3\), the final
discrete values after partition-wise argmax rounding are \(144.89\) (CG)
and \(143.63\) (\textit{ATCG})---a gap below \(1\%\)---confirming the
prediction of Theorem~III.1: restricting gradient evaluations to the
active sets \(\{\mathcal{A}_i\}\) via the \(\tau\)-coverage
rule~\eqref{eq:eta_def} introduces only a controlled approximation loss
relative to full~CG.


% \textbf{Objective quality (Fig.~\ref{fig:traj_cifar_atcg})} shows that \textit{ATCG} tracks CG throughout all $100$
% iterations without visible deviation and the final discrete values after
% partition-wise argmax rounding are $144.89$ (CG) and $143.63$
% (\textit{ATCG})---a gap below $1\%$---confirming the prediction of Theorem~III.1: restricting gradient
% evaluations to the active sets $\{\mathcal{A}_i\}$ via the $\tau$-coverage
% rule~\eqref{eq:eta_def} introduces only a controlled approximation loss
% relative to full~CG.



\textbf{Communication reduction (Fig.~\ref{fig:comm_cifar_atcg}).}
In contrast to CG and SCG \cite{mokhtari2018conditional}, whose communication grows steadily as $\mathbf{x}$
densifies, \textit{ATCG}'s cumulative upload curve bends over and becomes
completely flat well before the optimization terminates. This is the direct
signature of active-set stabilization, i.e., once every $\eta_i \geq \tau$, the
expansion rule in Algorithm~2 ceases to fire and no further feature
embeddings are sent to the server--yet the objective continues to improve on
the already-cached~information.



\begin{figure}[t]
\centering
\includegraphics[scale=0.3]{Fig/fig_tau_sweep_active_growth.png}
\caption{\reza{\small Total active-set size \(\sum_i|\mathcal{A}_i|\) versus iteration for
\textit{ATCG} with different threshold values \(\tau\). %Larger thresholds lead to larger active sets and higher communication.
}}
\label{fig:active_growth_cifar_atcg}\vspace{-0.2in}
\end{figure}


\textbf{Active-set dynamics (Fig.~\ref{fig:active_growth_cifar_atcg}).}
Figure~\ref{fig:active_growth_cifar_atcg} makes the communication cutoff
mechanistically transparent. \reza{In the early iterations, several partitions
have \(\eta_i < \tau\), so the expansion step in \textit{ATCG} fires and
\(\sum_i|\mathcal{A}_i|\) grows.} Once sufficiently informative candidates
are admitted, the partitions satisfy \(\eta_i \geq \tau\) and the curves
level off to constants. These plateaus directly correspond to the flat
regions of Fig.~\ref{fig:comm_cifar_atcg}: after stabilization,
optimization proceeds entirely on cached embeddings with zero additional
uploads. The plateau values \(\sum_i|\mathcal{A}_i| \ll |\mathcal{P}|\)
represent the total communication cost of \textit{ATCG}, consistent with
the communication bound established in Section~\ref{sec:algo_theory}.
Moreover, the different plateau values across \(\tau\) illustrate the
expected threshold-dependent tradeoff: larger \(\tau\) values impose a
stricter active-set coverage requirement and therefore activate more
elements, while still preserving objective values close to full~CG.


% \textbf{Active-set dynamics (Fig.~\ref{fig:active_growth_cifar_atcg}).}
% Figure~\ref{fig:active_growth_cifar_atcg} makes the communication cutoff
% mechanistically transparent. In the first $\sim\!50$ iterations, several
% partitions have $\eta_i < \tau$, so the expansion step (Algorithm~2, line~11)
% fires and $\sum_i|\mathcal{A}_i|$ grows. Once the most informative candidates
% are admitted, all partitions simultaneously satisfy $\eta_i \geq \tau$ and the
% curve levels off to a constant. This plateau directly corresponds to the flat
% region of Fig.~\ref{fig:comm_cifar_atcg}: after stabilization, optimization
% proceeds entirely on locally cached embeddings with zero additional uploads.
% The plateau value $\sum_i|\mathcal{A}_i| \ll |\mathcal{P}|$ is the
% communication cost of \textit{ATCG} in its entirety, consistent with the
% bound established in Section~\ref{sec:algo_theory} and further improved under
% the low-curvature guarantee of Theorem~III.2: the visual similarity shared
% across animal categories implies low total curvature $c$, so
% $\max\{\tau,\,1{-}c\}$ substantially exceeds $\tau$ and \textit{ATCG}
% approaches full CG performance with an even smaller active set than the
% threshold alone would require.


